Analysis of Independent Learning in Network Agents: A Packet Forwarding Use Case

Multi-Agent Reinforcement Learning (MARL) is nowadays widely used to solve real-world and complex decisions in various domains. While MARL can be categorized into independent and cooperative approaches, we consider the independent approach as a simple, more scalable, and less costly method for large-scale distributed systems, such as network packet forwarding. In this paper, we quantitatively and qualitatively assess the benefits of leveraging such independent agents learning approach, in particular IQL-based algorithm, for packet forwarding in computer networking, using the Named Data Networking (NDN) architecture as a driving example. We put multiple IQL-based forwarding strategies (IDQF) to the test and compare their performances against very basic forwarding schemes and simple topologies/traffic models to highlight major challenges and issues. We discuss the main issues related to the poor performance of IDQF and quantify the impact of these issues on isolation when training and testing the IDQF models under different model tuning parameters and network topologies/characteristics.

==> Analysis of Independent Learning in Network Agents-A Packet Forwarding Use Case/RL4NDN.tex <==
%\section{Multi-agent Reinforcement Learning for Intelligent Stateful Forwarding}
%\section{Intelligent Stateful Forwarding}
\section{IQL-based Stateful Forwarding}


\label{sec:RL}
%\textcolor{blue}{
In this section, we illustrate our IQL-based NDN forwarding scheme, IDQF where each node makes autonomous forwarding decisions based on their own observations and rewards. We also assess the performance of this scheme by comparing it to %a very basic state-of-the-art forwarding strategy such as 
the {\em best\_route} (BR)~\cite{yi2013case}.
%} 
%\textcolor{blue}{in a real-world network involving a number of routers and communication flows,  the size and complexity of state-action pairs can be very large, which poses a significant challenge for IQL to learn the optimal decision policy. To resolve this challenge in the IQL method, non-linear data driven model such as a neural networks are employed due to their ability to achieve generalization in the presence of multiple complex interactions.}


%----------------------------------
% Then, we need to talk about the following:
% \begin{itemize}
%     \item We have designed and implemented an RL forwarding scheme
%     \item We have tested and tuned many parameters, topologies, etc.

%     \item We compare to one of the most basic algorithms, bestroute (BR).

%     \item We use ndnSIM and plot results

%     \item describe results
% \end{itemize}

%----RL forwarding scheme--------
\subsection{Design of IDQF Forwarding Scheme}
%In the context of NDN, agents are deployed in each router that is responsible for making forwarding decisions for the Interest packets arriving at that router. 
The goal of the agent in each router is to autonomously learn a decision policy to forward Interest packets through the optimal next-hop interface. The schematics of the IDQF forwarding scheme
is shown in Figure~\ref{fig:rl-model-2}. The agent learns/discovers the optimal forwarding policy indirectly using the action-value function. %, that is approximated by a deep neural network and is referred to as Deep-Q-Network~(DQN)~\cite{mnih2015human}. 
In the vanilla Q-learning approach, the state-action pairs are mapped to corresponding Q-values (maximum expected rewards) by maintaining a Q-table. For a communication network with numerous routers and communication flows, the size and complexity of state-action pairs or the corresponding Q-table will be very large, which poses a significant challenge for IQL to learn the optimal decision policy. To resolve this, we  approximate the action-value function using neural networks and use the Deep-Q-Network (DQN) training algorithm~\cite{mnih2015human}.

%--------------------------
%This approach of Q-learning combined with the deep neural network is referred to as Deep-Q-Network~(DQN)~\cite{mnih2013playing}. 
%------------------
\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.99\linewidth]{rl-model-4}
  \caption{High level design of the IDQF forwarding strategy implemented at any router in the network. Periodically, routers update their states when receiving incoming Interests, and measure rewards when Data packets are received from the producer.  %{\abde This graph is not very clear to me. Arrows are still pointing to random places. Let's customize this example for the paper. Outcome must be the set of interfaces (face 1 and 2)}
  %[\textbf{If you agree with this caption, then remove color}]}
  }
  \label{fig:rl-model-2}
\end{figure}
%-----------------

As shown in Figure~\ref{fig:rl-model-2}, the router $RA$ is equipped with neural network DQN.
At decision time $t$, $RA$, calculates the state of its available next hop interfaces, \textit{Face1} and \textit{Face2} by observing some local parameters such as round trip times (RTTs), interest satisfaction ratios, number of re-transmitted packets collected between time $t$ and $t-\delta t$. Here, $\delta t$ is the time period for sensing and updating the weights of the DQN. The state is fed into the DQN as input. DQN then predicts either \textit{Face1} or \textit{Face2} as an action. The $RA$ agent then forwards the current Interest packet and all subsequent Interest packets through the predicted interface until next decision time occurs at $t+\delta t$. The chosen action results in a change of state for the corresponding interface. $RA$ also gets a feedback for its action, which is the reward. We define the reward, $RW(t)$ at time $t$ by the following equation: 
\begin{equation}
\label{eq:rw}
    RW(t) = -\Big[ \Big( \frac{1}{M}\sum_{k=(t-\delta t)}^t{RTT(k)} \Big) + C \times R(t) \Big]
\end{equation}
Here, $M$ is the number of Data packets received between $t$ and $t-\delta t$, %$RTT_k$ is the list of the received Data packets during the last period $\delta t$, 
$RTT(k)$ is the Round-Trip Time (RTT) of the received Data packet at time $k$, $R(t)$ is the number of re-transmitted packets which were actually transmitted through the interface chosen for the $\delta t$ period, and $C$ is a penalty constant multiplier that aims at discouraging choosing interface with high drop ratios (we choose $C=4$ seconds in our case). Note that in case of drops of Interests/Data packets, there will be no RTT measurements, thus the penalty constant helps in assigning a maximum delay for every packet dropped. % to assign penalty for the re-transmitted packets due to packet drops. 
%The negative sign is required in this case because DQN maximizes the reward and in our case the objective is to minimize the overall delay. 
The $RA$ agent uses the reward to improve its decision policy.

%%to work as an agent. When an Interest packet arrives at $RA$, it perceives the state for each of its available next hop interfaces, \emph{face1} and \emph{face2} by observing some local parameters such as RTTs, interest satisfaction ratios, number of re-transmitted packets. These parameters are fed into the DQN
%-------------------------
% Upon receipt of an Interest packet, $RA$, perceives the state of its available next hop interfaces, \emph{Face1} and \emph{Face2} by observing some local parameters such as RTTs, interest satisfaction ratios, number of re-transmitted packets. These parameters are fed into the DQN as input. DQN then predicts either \emph{Face1} or \emph{Face2} as an action. The RA agent then forwards the Interest packet through the calculated interface resulting in a change of state for the corresponding interface. It also gets a feedback for its action, which is the reward. The reward is designed as negative of the average RTT of Data packets received through the last chosen interface. The negative sign is required in this case because DQN maximizes the reward and in our case the objective is to minimize the overall delay. The RA agent uses the reward to improve its decision policy. When another Interest packet arrives at RA, the new states of the next hop interfaces are observed and a new decision is made. 

%---------------------------
%The reward function can be efficiently crafted to improve the network performance. In a simplistic scenario the reward function can be chosen to maximize the throughput and minimize the delay.
%====================================
%---------------
%The state space for the router agent comprises of three different statistics extracted from the Interest and the Data packet transmissions in the network. First statistic is the delay which  represents the time duration between an Interest packet is sent and its corresponding Data packet is received, and is also referred to as round-trip time (RTT). 
%------------------------
%High RTT corresponds to high traffic in the network. 
%---------------------------
%Second indicator of the network state is a re-transmitted Interest packet. When no Data packet is received for an Interest packet within a certain period of time, another Interest packet with the same name is requested by the client.  This Interest packet is denoted as the re-transmitted packet which represents the congested scenario of the network. Third is the Interest Satisfaction Ratio (\emph{ISR}) that is defined by the ratio of the number of Data packets received through a next hop interface and the number of Interest packets sent through that interface in the last decision epoch. High \emph{ISR} value stands for low congestion in the network. All these statistics are extracted at a decision epoch for every next-hop interfaces that are connected to a particular router, $r$, where the RL agent is deployed. 

%The action space of the router agent, $r$ is the set of available next hop interfaces. Once the router agent, $r$ predicts an interface as an action, it forwards $\delta t$ Interest packets through that chosen interface, before a new decision is made. The reward function can be designed to minimize the overall delay. We define $R$ to be the number of re-transmitted packets and $N$ to be the number of new packets in the last decision epoch. Let us define the reward function as: $-(AvgD + R_{lf}\times CM)$, where $lf$ is the chosen interface in the last decision epoch, $R_{lf}$ is the number of packets in $R$ which were transmitted through $lf$ last time, $AvgD$ is average of delay of the data packets received through interface $lf$ between last decision epoch and current decision epoch, $CM$ is a constant multiplier to assign penalty for the re-transmitted packets due to packet drops. 

%\todo[inline]{TODO: further summarize}

%=============================

%\subsection{Simulation Results}
\subsection{Evaluation of IDQF}
We use \emph{ndnSIM}~\cite{mastorakis2017ndnsim}, the NDN network simulator, to evaluate the forwarding scheme performance. %Our proposed RL forwarding scheme is implemented as a daemon process that interfaces with the \emph{ndnSIM}. 
To implement the RL agents, % in nodes of the simulator, 
we used a concurrently running daemon process that interfaces with the \emph{ndnSIM} and exchanges training data and prediction of the next hop interface for each node. In this paper, we will share the results using the Sprint topology shown in Figure~\ref{fig:topo-Sprint-2}. We have  tested the performance using multiple network topologies (grid, tree), and performed tuning of different parameters of DQN.
%\todo[inline]{talk more about examples of tuning that we tested. Be concise.}

%\todo[inline]{TODO: reduce white space in figure and increase font as much as possible.}

\begin{figure}[htbp]
  \centering
  %\includegraphics[width=\textwidth,height=8cm]{figures/sprint2-wcp.pdf}
  \includegraphics[width=0.9\linewidth]{figures/sprint-2-ann-final.pdf}
  %\includegraphics[scale=.5]{figures/SPRINT_marked_v1.pdf}
  \caption{Sprint topology used in our simulation; propagation delays (in milliseconds) are shown as link weights; link capacities vary from 1Mbps at the core (black links), 2Mbps (grey) and 5Mbps at the edge (blue)} 
  \label{fig:topo-Sprint-2}
\end{figure}

We consider a simple scenario, where only one consumer ($C_0$) requests data from only one producer ($P_0$) at a fixed rate $r$. Note that we used such a simple scenario to highlight challenges that may arise even in a very predictable network traffic with no loss, errors, contention, etc. 
The Sprint topology in Figure~\ref{fig:topo-Sprint-2} consists of $11$ router nodes and $18$ links among them. %The bandwidth and delays (in milliseconds unit) of each link are labeled in Figure~\ref{fig:topo-Sprint-2}.
%Every node in the network can hold maximum 100 packets in the transmission queue. 
Each router node has a queue size of 100 packets. 
In our simple scenario, we deploy the agents in nodes $N_3$, $N_4$, $N_6$, and $N_9$ only. Each of these agents have their own IDQF-strategy.  %To reduce the computational complexity, we also limit the action space of each agent to two, that is, there will be only two interfaces available for forwarding of each Interest packet.
In our results, we have considered the size of the state vector to be two and chose the best two interfaces at each agent (those with the least delays to the producer). Note that we have used and tested different sizes which result in performance degradation when we scale the exploration beyond two interfaces. % and results Since in forwarding strategy, our main goal is to efficiently utilize the interfaces already ranked by routing protocols, we are more interested in assessing the performance of 2 best interfaces rather than using all the available interfaces. That is why, we limit the action space of each agent to two.}  

In our simulations, the DQN of each agent has one hidden layer, one input layer and one output layer. Each hidden layer
consists of 32 nodes, and the layers are fully connected with
each other.
While training the node agents we tuned several parameters of DQN. The first parameter is the decay rate, which controls the number of times the agents will perform exploration by randomly choosing actions. Second, we adjusted the learning rate to control the convergence speed of DQN. Third, we varied the capacity of the replay buffer which governs the diversity of samples available to the agent at any moment. 
%Fourth, we trained the agents for different number of episodes where an episode corresponds to one instance of simulation of the network environment. Finally, we considered short (30s) verses long duration (120s) of simulation per episode while training the agents. 
%-----------------------------

%The parameters are briefly described below.
%\begin{enumerate}
    %\item \textbf{Exploration rate:} It is necessary to trade-off between exploration and exploitation of the environment in any RL algorithm. We adopted decaying epsilon-greedy method in our experiments. In this method, we utilized the decay rate, $\lambda$ to control the number of times the agents will perform exploration by randomly choosing actions. As the agent learns more about the environment, the decay rate will allow the exploration to be reduced progressively so that the agent can exploit knowledge from the deep neural network and take actions. In our experiments, we tested $\lambda$ with values $0.1, 0.01, 0.001,$ and $0.0001$. 
    
    %\item \textbf{Learning rate:} In deep neural network, learning rate, $\eta$ controls how quickly the optimization will converge. While training and deploying the RL agents, learning rate can effect the decision policy of the agents.During training, small learning rate is needed for the agents to change policies slowly and reach an optimal policy at the end of many iterations. However, the agents also learn in deployment mode and requires changing policy quickly to adapt to the dynamics of the environment. We kept the learning rate parameter value to 1.0 during training and varied it with 1, 100, and 500 in deployment mode of the agents.   %------------------------------ 
    %%keeping the learning rate too small during training can cause the optimization to take a lot of time to converge. On the other hand, if learning rate is too large, then training may not converge or even diverge because big weight changes will let the optimizer overshoots the minimum and thus making the loss worse. 
    %-----------------------------
    %\item \textbf{Replay buffer size:} Experience replay memory in DQN holds transition samples from agent's prior and recent behaviors. The size of the replay buffer governs the diversity of samples available to the agent at any moment. This diversity can affect the learning behavior of the agents. We altered the capacity of the replay buffer to find the performance improvement and the impact on policy learning of our agents. We used replay buffer size of 600, 1200, 1800, and 2400 in our experiments.
    
    %\item \textbf{Number of episodes:} In our experiments, we consider one instance of simulation of the network environment an episode. During training the number of episodes may have an impact on the policy learning of the agents. We considered setting the number of episodes to 1, 30, 50 and 100 in our experiments. 
    
    %\item \textbf{Episodic duration:} In RL algorithm, the number of time steps in one episode may play a role in how well the agents will learn. In our case,  we can't set any fixed number of time steps per episode because it will depend on the request rate of the client in the simulation environment. However, we can control the duration of the network simulation since each simulation is considered as an episode. In our experiments, we tried short (30s) verses long duration (120s) of simulation while training the agents.    
    
%\end{enumerate}
%\todo[inline]{Too long. We need at most one paragraph for all}
%-------------------------------
%We share the results obtained when we configure and train the RL model using %{\abde .... continue without using the variables, also no need to list the rates}...
We trained the DQN of agents with decay rate=$0.001$ and learning rate=$1.0$ for 50 episodes where an episode corresponds to one instance of simulation of the network environment with duration 60 seconds. The agents were trained separately for five different request rate starting from low Interest rate (41\% of network capacity) to high Interest rate (123\% of network capacity) in packets/second (pkts/s). The interest rates are 100 pkts/s (0.82 Mbps), 150 pkts/s (1.23 Mbps), 200 pkts/s (1.64 Mbps), 250 pkts/s (2.05 Mbps), and 300 pkts/s (2.46 Mbps). We deployed the agents for each Interest rate and ran simulations five times to get average results.
%\textcolor{red}{Write about data rate in Mbps and what percentage of network capacity?}
%of 100 (0.82 Mbps), 200 (1.64 Mbps), 300 (2.46 Mbps), 400 (3.28Mbps) and 500 (4.09 Mbps) interests per second. 
We compare the throughput and average delay measured in $C_0$ for both BR and IDQF scheme and present the results in Figure~\ref{fig:thrpt-del-comp}. 
The height of the bar for each point in Figure~\ref{fig:thrpt-del-comp} represents the standard deviation of throughput and delay measurements at every second of simulation.  
%----------------------------
\begin{figure}[!th]
\begin{subfigure}{0.46\columnwidth}
\centering
\includegraphics[width=\linewidth]{./figures/RtCmpAvg-thrpt-rt=0.pdf}
\caption{Throughput measurements at the consumer node $C_0$}
\label{fig:thrpt-comp}
\end{subfigure}
\begin{subfigure}{0.46\columnwidth}
\centering
\includegraphics[width=\linewidth]{./figures/RtCmpAvg-delay-rt=0.pdf}
\caption{End-to-end delay measurements at the consumer node $C_0$}
\label{fig:delay-comp}
\end{subfigure}
\caption{Throughput and delay comparison of \emph{best\_route} (BR) and IDQF performance; Error bars indicate the variation of the measurements during the simulation} 
\label{fig:thrpt-del-comp}
\end{figure}
%-----------------------------
%From Figure~\ref{fig:thrpt-comp}, we find that the throughput of BR strategy starts decreasing when the data rate is greater than 2.45 Mbps which is more than the 2 Mbps network capacity. Though the throughput of RL strategy is not as good as BR strategy for lower data rates, we observe 25.21\% and 15.27\% throughput improvement of RL over BR for 3.28 Mbps and 4.09 Mbps data rates respectively. Similarly, in Figure~\ref{fig:thrpt-del-comp}, we find 14.5\% and 7\% reduction in average application delay of RL over BR for 3.28 Mbps and 4.09 Mbps data rates respectively. %--------------------------

%\textcolor{red}{ADD OPTIMAL THROUGHPUT AND DELAY in the Figure and ADD TEXT}
Figure~\ref{fig:thrpt-del-comp} shows that the IDQF strategy does not outperform even the most basic %state-of-the-art 
strategy, {\em best\_route} (BR). BR always uses the interface with the shortest delay regardless of congestion. It will react and switch an interface only if the best route fails (after at least one timeout event). Note that we share the IDQF configuration that provides the best results for this scenario. 
As shown in Figure~\ref{fig:thrpt-comp}, BR outperforms IDQF by 10\%-36\% in terms of throughput for all Interest rates. We notice that IDQF often fails to choose the best interface, provided the cost (\eg latency from the router to the producer) of using each interface. %to reach the producer. 
%%Other (smarter) forwarding strategies, \eg AFS, {\abde add more}, are able to perform better in high congestion scenario.
%-------------------------
% First, BR outperforms IDQF for smaller Interest rates. We notice that IDQF often fails to choose the best interface, provided the cost (\eg latency from the router to the producer) of using each interface. %to reach the producer. 
% Second, while IDQF slightly outperforms BR at larger Interest rates, the performance difference remains less than 10\%. 
%%Other (smarter) forwarding strategies, \eg AFS, {\abde add more}, are able to perform better in high congestion scenario. 
Similarly, in Figure~\ref{fig:delay-comp}, we find that IDQF strategy fails to deliver data faster than BR in most cases, especially at lower Interest rates. Interests are often forwarded to interfaces that lead to congestion and drops, resulting in an average of 2 to 3 re-transmissions per Interest. 

To summarize, IDQF strategy, while tested even with a simple scenario with a single flow and limited network variability, fails to converge into a stable state that learns the non-changing network characteristics and makes decisions that can often be solved by simple utility functions. 
In this study, we have identified a list of challenges (discussed in the next section) which advocate that reinforcement learning based approaches driven by autonomous decision making paradigm will result in similar non-optimal or sub-optimal solutions. These challenges are generalized beyond NDN, and may apply to IP and other network architectures/systems.
%but also in IP network in general. In the next section, we try to list and discuss the major challenges that contributed in the IDQF strategy failure(s) and do exist in all independent decision making based approaches. }

%Next, we will list and discuss the major challenges that contributed in the IDQF strategy failure(s). 

==> Analysis of Independent Learning in Network Agents-A Packet Forwarding Use Case/abstract.tex <==
\begin{abstract}
%\textbf{***OLD TEXT***}
% One of the main features of %Named Data Networking (NDN) 
% Information Centric Networking (ICN) is stateful forwarding, which enables routers to maintain a state of all pending Interests to better guide data packets back to the consumers. Stateful forwarding can be used to help adapt to network changes, load balancing, and improve Quality of Service (QoS).{\abde I wouldn't start with ICN. Even title doesn't have ICN. I suggest we use the same story of the intro, just summarize it}
% %However, stateful forwarding can also be used to help adapt to network changes, load balancing, and improve Quality of Service (QoS). 
% %In this article, we discuss the potentials and challenges associated with intelligent stateful forwarding based on multi-agent reinforcement learning. 
% In this paper, we implemented a forwarding strategy, IDQF by adopting one of the multi-agent reinforcement learning approaches. The goal of IDQF is to obtain optimal network performance by having routers dynamically learn complex network characteristics and choosing the most suitable interface to forward Interest packets. We evaluate IDQF's performance against a basic forwarding strategy, \textit{best\_route} in NDN architecture and discuss the potentials and challenges of the forwarding problem in the distributed multi-agent scenario. 
%=============================================
%Multi-agent reinforcement learning is nowadays widely used to solve real-world and complex decisions in variety of domains where multiple autonomous agents are needed to better sense the environment and/or make  decisions independently. 
%----------------------------------------
Multi-Agent Reinforcement Learning (MARL) is nowadays widely used to solve real-world and complex decisions in various domains. While MARL can be categorized into independent and cooperative approaches, we consider the independent approach as a simple, more scalable, and less costly method for large-scale distributed systems, such as network packet forwarding. % is the most appealing in terms of scalability and communication efficiency. 
%In autonomous agents approach, multiple agents locally sense their shared environment and/or make  decisions independently. 
In this paper, we quantitatively and qualitatively assess the benefits of leveraging such independent agents learning approach, in particular IQL-based algorithm, for packet forwarding in computer networking, using the Named Data Networking (NDN) architecture as a driving example. We put multiple IQL-based forwarding strategies (IDQF) to the test and compare their performances against very basic forwarding schemes and simple topologies/traffic models to highlight major challenges and issues. %and studied the impact of different model tuning parameters and network topologies/characteristics. We use a real-world network topology, and compare against one of the basic forwarding strategies, \textit{best\_route}, to highlight some of the challenges of IDQF agents. 
We discuss the main issues related to the poor performance of IDQF, and quantify the impact of these issues on isolation when training and testing the IDQF models under different model tuning parameters and network topologies/characteristics.   %We discuss four important challenges of IDQF in particular, and autonomous multi-agent reinforcement learning approaches in general, when applied to the packet forwarding use-case. 
%We argue that some of these challenges may apply to other scenarios, such as distributed robotics, and if not adequately addressed can lead to major performance degradation.   


% physically sca, including robotics, distributed control, etc. Despite applications in various fields, very few multi-agent RL algorithms have been evaluated in distributed networking environment. In this paper, we adopted the forwarding decision problem in NDN architecture as a model for assessing one of the multi-agent reinforcement learning approaches, IQL. We implemented a forwarding strategy, IDQF using that approach and evaluated its performance against a basic forwarding strategy, \textit{best\_route} available in NDN. We also focus on raising some practical challenges of this approach in such distributed environment.    


%===========END===================
%we discuss the challenges pertaining to observation of network states, choice of reward functions, and convergence in the distributed multi-agent scenario.
%------------------------
%In this paper, we consider a reinforcement learning (RL) approach to highlight the benefits of stateful forwarding in ICN. We propose, \sol that implements an RL algorithm to dynamically learn complex network characteristics and chooses the most suitable interface to forward Data packets such that the award is maximized. 
%without the necessity of labeled training data. The ability of the RL to make short term decisions with the objective to optimize a longer term goal makes it a perfect candidate for packet forwarding in the NDN. The RL may yield superior routing performance in NDN by appropriate parametric calibration of the ML loss function or the objective function. 
%----------------------------
%We implement and evaluate \sol, our generalized RL-based solution approach. \sol achieves a better delay throughput tradeoff, when compared to state-of-the-art \emph{Best route} strategy, with up to 55\% higher throughput and 30\% shorter delay measurements. 
%----------------------------
%The goal of this paper is to assess the performance of Machine Learning (ML) algorithms such as Reinforcement Learning (RL) for intelligent packet forwarding in NDN. The RL algorithms can learn complex system behaviors without the necessity of labeled training data. The ability of the RL to make short term decisions with the objective to optimize a longer term goal makes it a perfect candidate for packet forwarding in the NDN. The RL may yield superior forwarding performance in NDN by appropriate parametric calibration of the state and objective function. In this paper, we attempt to unveil the effect of the parameters and evaluate a generalized RL based solution approach by comparing the performance with the state-of-the-art \emph{Best route} strategy, which is default in \emph{ndnSIM}.
\end{abstract}


==> Analysis of Independent Learning in Network Agents-A Packet Forwarding Use Case/background.tex <==
\section{Background And Related Work}
\label{sec:motiv}


%============================
%\subsection{Reinforcement Learning}
%\label{subsec:rl}
%\todo[inline]{Copied from old text. We need to summarize and simplify}
%In control theory, the Markov Decision Processes (MDP) are a set of standard formalism to solve sequential decision making problems, where the control actions determine the evolution of the state of the system. 
 %at discrete time step. 
%% The RL is a specific family of the finite horizon MDPs with guarantee of convergence. %The state, action, policy, and reward together define a MDP. . Bellman equation.
%% Under a standard RL~\cite{sutton1998introduction} setting, 
%The decision making module (also refereed as the agent) in an MDP interacts with an environment in every discrete decision epochs. 
%----------content-------------------
% RL is typically formalized using the Markov Decision Process (MDP) which can be viewed as a model of an agent that interacts with an environment to solve decision making problems.
% At each decision step $t$, the agent observes a state $\mathbf{S}_t$ of the environment and takes an action $\mathbf{A}_t$ according to a policy $\pi(\mathbf{S})$. After taking the action, %the environment assigns 
% the agent receives a reward $R_t$ and the environmental state evolves to $\mathbf{S}_{t+1}$. % and the agent receives a reward $R_t$. 
% The goal of the agent is to find an optimal policy $\pi^*(\mathbf{S})$ that maps its state to either a deterministic action or a probability distribution over actions so that the over-all cumulative reward, % at time $t$, 
% $R_t(\mathbf{S}_t, \mathbf{A}_t)$ %$\sum_{t=0}^{t=T} R(\mathbf{S}_t, \mathbf{A}_t)$
% is maximized.
% The term $R_t(.)$ represents the reward function, that is dependant on the input states of the environment and the actions of the agent. % and $\gamma \in [0,1]$ is the factor that discounts future rewards.
% %$\sum_{t=0}^{t=T}\gamma^t R(\mathbf{S}_t, \mathbf{A}_t)$ 
% When the system model is known, the optimal policy of an MDP can be computed using dynamic programming. However, in most real world applications such as in our problem of stateful forwarding, the system model is unknown. %RL is a specific approach for computing the optimal policy for an MDP when the model is unknown. 
% %The RL algorithms address this class of MDPs. 
% To address this class of MDP, one of the promising approaches for RL is to use model-free algorithms which estimate optimal policy directly from experience and without knowing the dynamics of the environment. In this article, we focus on a value-function based approach to deal with packet forwarding.
%===================================
%\subsection{Reinforcement Learning}
%\label{subsec:rl}
%\textcolor{red}{@Abu: Lets define reinforcement learning first and then briefly describe what it does and how is it used in a scenario with multiple RL agents. Describe IQL, MDP. Why IQL and not the other centralized approach.} 
%---------------------------------
%In a single agent environment, 
% Reinforcement Learning is typically formalized using the Markov Decision Process which can be viewed as an interaction process of the agent to solve decision making problems. At each decision step, the agent observes a state of the environment and takes an action according to a policy which is a mapping from states to actions. After taking the action, the agent receives a reward and the environmental state evolves to a new state. The goal of the agent is to find an optimal policy that maximizes the over-all cumulative reward. In most real world applications such as in our problem of stateful forwarding, the system model is continuously evolving and unknown. To solve this class of Markov Decision Process, one of the promising approaches for RL is to use model-free algorithms such as Q-learning~\cite{watkins1992q}. In Q-learning, the value of taking an action in a state is formalized using an action-value function. An iterative method is then applied to learn the optimal action-value function and use it to find the optimal policy. 

%In this article, we focus on a value-function based approach to deal with packet forwarding.
%---------------------------------

%\textcolor{blue}{
% In multi-agent environments, one of the straightforward RL approaches is to train a joint model through centralized learning from the combination of observations and actions of all agents. In this approach, a central controller forms a joint state by concatenating states of all agents and outputs a joint action policy for all agents. A major drawback of this approach from the perspective of forwarding is scalability because the sizes of observations and action spaces grow exponentially with the number of agents or network routers. Besides, %in many real-world applications 
% it is inefficient for a central controller to have full observability of the environment and take actions for all agents. 
% To deal with these issues, a preferred approach is decentralized learning, where each agent is trained independently from others and takes autonomous decisions. %for itself. 
%----------------------------
% Two broad categories of decentralized learning approaches exist in the literature for multi-agent environment: cooperative agents and independent agents. 

% In the cooperative agents category, agents cooperate with each other through communication to have access to the observations, actions, and rewards of other agents~\cite{gupta2017cooperative}. We argue that in addition to communication cost, the cooperative agents approach also suffers from some challenges such as coordination problem (\eg coherently choosing individual actions of all agents such that the resulting joint action is optimal) and credit assignment problem (\eg estimating each agents contribution to generating global reward).
% %\textcolor{blue}{As communication networks continue to expand and become more complex day by day, using a central entity similar to SDN for packet forwarding turns out to be an infeasible solution. A more scalable and efficient solution is to allow each router in the network to use localized information to make forwarding decisions and try to optimize the network performance.}

% The independent agents category or IQL is an approach where each agent exclusively uses its own history of partial observations and local rewards to learn, and considers other agents as part of the environment~\cite{wei2019presslight}. 
% %This category of RL emerges as the most appropriate approach for our goal of intelligent stateful forwarding.
% In IQL, to handle the increased state-action pairs encountered in packet forwarding, due to the network dynamics a neural network is used. 
%-------------------------------------
% A limitation of the IQL is that each agent runs a separate Q-learning algorithm. As a result, the size and complexity of the Q-table may increase enormously for state-action pairs encountered in our problem of packet forwarding, due to the network dynamics. This poses a significant challenge to learn the optimal policy. A deep neural network, due to its ability to achieve generalization in the presence of multiple complex interactions, is deployed to resolve this challenge and learn the optimal policy by approximating the dynamic action-value function. 

%This approach of IQL combined with the deep neural network is referred to as Deep-Q-Network~(DQN)~\cite{mnih2013playing}. 
%---------------------
%In this paper, we limit our focus on the IQL approach with deep neural networks to address the packet forwarding problem and refer to the forwarding strategy as IDQF.
%-------------------------
%and lacks the global information. 
%While IQL method has its limitations due to lack of global information and a cooperation mechanism, it has been successfully applied to solve air traffic flow control problem~\cite{agogino2012multiagent}. %and has the benefit that the size of the state-action space is linear with the number of agents. 
%However, the increase in size and complexity of the Q-table, pose significant challenge for the IQL to learn the optimal policy. A neural network, due to its ability to achieve generalization in the presence of multiple complex interactions, is deployed to resolve this challenge and learns the optimal policy by approximating the action-value function. %have the ability to learn the optimal policy solve this have proven have the ability to  and availability of sufficient training data. %--------------------------
%In this paper, we focus on IQL based approach to address our packet forwarding problem in networks. %Since Q-learning increases storage complexity with the increase of problem size, in our IQL approach we employ neural networks to approximate the action-value function.  
%While IQL method has its limitations due to lack of global information and a cooperation mechanism, it has been successfully applied in some domains~\cite{agogino2012multiagent} and has the benefit that the size of the state-action space is linear with the number of agents. We argue that in addition to communication cost, the cooperative agents approach also suffers from some challenges such as coordination problem (\eg coherently choosing individual actions of all agents such that the resulting joint action is optimal) and credit assignment problem (\eg estimating each agents contribution to generating global reward). Therefore, in this paper we focus on IQL based approach to address our packet forwarding problem in networks. Since Q-learning increases storage complexity with the increase of problem size, in our IQL approach we employ neural networks to approximate the action-value function.  

%===========================
%In addition to communication cost, this approach suffers from coordination problem (\eg coherently choosing individual actions of all agents such that the resulting joint action is optimal) and credit assignment problem (\eg estimating each agents contribution to generating global reward). Since IQL method has been successfully applied in some domains~\cite{agogino2012multiagent} and has the benefit that the size of the state-action space is linear with the number of agents, in this paper we focus on IQL based approach to address our packet forwarding problem in networks. Since Q-learning increases storage complexity with the increase of problem size, in our IQL approach we employ neural networks to approximate the action-value function.
%}

\subsection{ICN/NDN Background}
\label{subsec:ndn}
Different from IP networks that use IP addresses (hosts identities) to inform intermediate routers' forwarding decisions, the fundamental idea of Named Data Networking (NDN) architecture is to retrieve the named-pieces of information (named network-layer packets), from any node that can provide it. 
%This ICN paradigm aligns network operations with the consumer/producer nature of edge-driven applications. 
In NDN, routers are equipped with a content store (CS), a pending interest table (PIT), and a forwarding information base (FIB). 
The FIB (similar to the forwarding table in IP routers) 
gets populated using a routing algorithm. 
Any node/router that receives a special packet (known as Interest packet) requesting for a content (Data packet) 
performs a CS-lookup on the content name. If the content is not available in the CS, the router performs a lookup in its PIT to check whether there is an existing request for the content that the router has forwarded into the network. 
If the PIT lookup is successful, the router adds the incoming Interest packet's interface to the PIT entry (interest aggregation) and drops the Interest. 
%If no PIT match is found, the router creates a new PIT entry for the interest and forwards the interest on the best interface(s) obtained from the FIB to an upstream router(s) in the direction of the data source(s). 
If no PIT match is found, the router creates a new PIT entry for the Interest. It then utilizes a forwarding strategy to select the best interface to upstream router(s) from multiple interfaces obtained from the FIB and forwards the Interest packet in the direction of the data source(s). 
%==================
%{\abde We must add here related work of RL-based techniques in NDN. Abu, I remember you have written this somewhere. We need to talk about these and highlight their limitations (\eg tested in simple topologies (the workshop paper is limited to one agent only if I remember well), or other limitations)}
%--------------------------

%{\bf Related Work:}
\subsection{Related Work}
There exists a good number of literature which applied RL to routing in networks~\cite{mammeri2019reinforcement}. We mainly outline a few research works that applied RL for designing forwarding strategies in NDN. 
In~\cite{chiocchetti2013inform,zhang2020afsndn}, authors proposed Q-routing based strategies that alternates between exploration and exploitation phases to learn the best interface in terms of a cost (\textit{e.g.} delay) during dynamic network conditions. However, the switching of the phases are dependent on some parameters and hampers the ability of the strategies to react quickly to network changes such as congestion. Moreover, it requires altering the default NDN packet formats and data structures to calculate experience information for Q-routing, which violates the principle of
data immutability in NDN. %Even though INFORM was evaluated on a Erdos-Renyi model based topology where each node had cache, it was never tested in a topology where no cache is present in the routers. 
%------------------------
%INFORM mainly aims at discovering the path to transient copies of content items rather than handling congestion in the network. 
%---------------------------
%It works well when content items from producer are cached in different nodes, but due to its slow reaction it performs poorly when there is no caching in the network and data rate is higher than the network bandwidth. 
%-----------------------------------
%Similar to INFORM, authors in~\cite{fu2017reinforcement}, used modified Q-routing to design a forwarding strategy. However, the strategy requires altering the default NDN packet formats and data structures to calculate experience information for Q-routing. Moreover, because of the slow learning of Q-routing, it is less adaptive to the changes in a network.
%------
%Another research work~\cite{ zhang2018ifs} 
The works~\cite{zhang2018ifs} and~\cite{de2020dqn} exploited neural networks to learn the mapping from the state of the network condition to the action of choosing the optimal interface for forwarding interests. However, there is no balancing of load across interfaces. Moreover, the strategies were verified using a single agent topology, which makes it difficult to assess the efficacy in larger/real networks.  
%However,this work fails to load balance between different interfaces. Moreover, rather than testing in a real network scenario, the authors evaluated their algorithm on a toy topology with a single node, which raises the question of the algorithm's effectiveness on real-world topologies in a multi-agent distributed scenario.  

==> Analysis of Independent Learning in Network Agents-A Packet Forwarding Use Case/challenges.tex <==
%\section{Research challenges}
\section{Challenges of using autonomous agents in distributed systems}
\label{sec:challenge}
%\textcolor{red}{List the key challenges and define them}
\textcolor{black}{We will build on the results shown in the previous section that highlight the sub-optimal performance of the IDQF strategy, and autonomous multi-agent RL algorithms in general.} In this section, we will discuss and analyze qualitatively and quantitatively few challenges that contribute to this ``low'' performance. 


%can be attributed to a variety of factors. In the following sub-sections, we summarize the  major challenges associated with multi-agent RL forwarding.
% In this section, we mainly list several challenges of DQN reinforcement learning algorithm in the context of our problem of designing a forwarding strategy in NDN network environment with multiple node agents.

\subsection{Training and Generalization of Agents}
The exhaustiveness of the sample training set and the method of training play a significant role in proper generalization of the neural network of an agent. In a multi-agent setting, the goal of every agent is to maximize its cumulative reward or the expected return, %.The expected return 
which is simply the sum of all rewards the agent received starting from the initial state to a terminal state of the environment. An agent can reach a terminal state if certain score is obtained or the task is complete. %The learning of an optimized policy works if we know what return to expect and train the agents iteratively by resetting the state to the initial state and start new agent-environment interaction. 
To learn an optimized policy the agents are iteratively trained through multiple episodes where each episode is a sequence of states, actions, and rewards starting from an initial state to a terminal state. Often, it is difficult to determine a terminal state or a target score for the network environment. 
%The sequence of states, actions, and rewards starting from an initial state to a terminal state is known as episode. Thus, the agents are iteratively trained through multiple episodes. Often, it is difficult to determine a terminal state or a target score for the network environment.  
%%So to make a final time step or terminal state we consider running a simulation for a specific period of time and call it a episode.
Therefore, we argue that setting the episode as a period of time, which is long enough to incorporate actions, and their rewards, will depend on the network topology and its characteristics (traffic, congestion). Based on the choice of episode length (simulation duration), there is a possibility of over-fitting or under-fitting of the neural networks of the agents, that can often lead to bad generalization and sub-optimal policy learning for the agents. 
%{\abde If we can find an optimal policy then there is no challenge! I was expecting that you complete the sentence by describing the challenge}.

%{\abde PLEASE COMPLETE THIS SENTENCE}.
%of time which is long we run the network simulation for a specific period of time and consider it as an episode. After each simulation ends, the agents will gather a cumulative reward which is the negative of the average RTT, in our context. The goal of each agent is to maximize its reward over one run of the simulation (episode) to reach an optimal policy after certain episodes.}
%---------------------------
% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.90\linewidth]{ep-vs-rw-duration-Node3}
%   \caption{Cumulative reward of node agent $N_3$ when trained for different duration of simulation  
%   }
%   \label{fig:duration-N3}
% \end{figure}
%--------------------------

To better illustrate this challenge, let us consider the scenario depicted in Figure~\ref{fig:topo-Sprint-2}. Agents closer to the consumer node would receive much more Interest packets, resulting in more data points, when compared to others closer to the producer node. Indeed, agents explore their interfaces by spreading received Interests across their next hop nodes, resulting in fewer number of Interests received by core routers which render learning more challenging at these nodes. 
For instance, nodes such as $N_4$ will not get enough number of Interests to build its training data within the short simulation duration. In our controlled experiments with a fixed network topology, we tested and tuned different simulation periods, yet failed to find optimal forwarding strategies for the nodes.

%assume that consumer is requesting with a low rate of 100 interests/sec and the episode length is 10s. In this scenario, the number of interests received by $N_9$ will be less compared to $N_3$. \textcolor{blue}{Because $N_3$ is the first node to receive all the interests sent by the consumer and will explore its outgoing interfaces by distributing those interests. Some of those interests will be received by node $N_9$. Now, $N_9$ will spread its received interests between its next hop nodes $N_8$ and $N_4$ while it is exploring. This will cause the original interests from the consumer to be further distributed.} As a result, nodes such as $N_4$ will not get enough number of interests to build its training data within the short simulation duration. In our controlled experiments with a fixed network topology, we tested and tuned different simulation periods, yet failed to find optimal forwarding strategies for the nodes. }
%--------------------------
%To provide an example for this challenge, let us assume that consumer is requesting with a low rate of 100 interests/sec and the episode length is 10s. In this scenario, the number of interests received by $N_9$ will be less compared to $N_3$. While $N_9$ is exploring, those interests will be further distributed among its next hops. As a result, nodes such as $N_4$ will not get enough number of interests to build its training data within the short simulation duration. In our controlled experiments with a fixed network topology, we tested and tuned different simulation periods, yet failed to find optimal forwarding strategies for the nodes.  
%---------------------------

%While the optimal period of time set as an episode varies based on the topology of the network, traffic, and the network congestion, our tests/tuning of these periods in controlled experiments did not lead to optimal forwarding strategies. 

%For instance, assume that after training $N_3$ learned that face leading to $N_9$ is its best strategy, when consumer node sends interests at 200 interests/sec, instantaneous congestion (\ie leading to drops) may occur, but $N_3$'s strategy will not react fast enough 
%(\textbf{CAN WE SAY HOW IS THIS RELATED TO TRAINING AND EPISODE PERIODS?})

%--------Replay buffer--------------
% During learning, instead of utilizing experience data (\ie state transition record as tuple $<$state, action, reward, next state$>$) for training immediately, the agent collects and stores the records in a circular memory buffer called \emph{experience replay} and update the weights of the DQN by randomly sampling mini-batches from it. The \emph{experience replay} technique helps the DQN to break correlation in observation sequences and learn from more independently and identically distributed past experience~\cite{mnih2015human} to stabilise the training. 
% The size of the \emph{experience replay} memory can influence the quality of learning of the resulting agent. %may cause bias in the function approximation estimate
% If the size of the \emph{experience replay} is large, then sometimes the recently experienced transitions will only be used for learning hundreds of steps later. Meanwhile, very old transitions, generated using an initially bad policy, can be used to train the network~\cite{zhang2017deeper}.
%-----------------------
%The training set for an agent also depends on the replay buffer~\cite{mnih2015human} that is used to store experience data (\ie state transition record as tuple $<$state, action, reward, next state$>$). Without replay buffer, agents will update the weights of their neural networks based on only current state, action and reward. However, sometimes state transitions generated by a good policy need to be saved to sample later for updating the neural network weights. 
%-----------Figure-4------------------
% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.90\linewidth]{ep-vs-rw-rp-2-Node3}
%   \caption{Cumulative reward of node agent $N_3$ with different sizes of replay buffer  
%   }
%   \label{fig:reply-buff-N3}
% \end{figure}
%------------------------------
The generalization of the agents also depends on the size of a memory buffer called \emph{experience replay}~\cite{mnih2015human} that is used to store experience data (\ie state transition record as tuple $<$state, action, reward, next state$>$). This replay buffer helps the neural networks to break correlation in observation sequences and learn from more independently and identically distributed past experiences to stabilise the training. Without replay buffer, agents will update the weights of their neural networks based on only current state, action, and reward. However, sometimes state transition tuples generated at earlier stage of exploration constitute a good policy for the agent. These records need to be stored and can be utilized for training the neural network to achieve better generalization. During training with replay buffer, the agents update the weights of their neural networks or DQN by randomly sampling mini-batches of experience data from it. 

To demonstrate the effect of replay buffer, we ran two experiments: one involving agents trained without any replay buffer and another by training agents with replay buffer. We show the cumulative rewards obtained by node agent $N_3$ per episode of training in Figure~\ref{fig:reply-buff-N3}.
%--------Figures---------------- 
%----------------------------
\begin{figure*}[tbp]
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{./figures/ep-vs-rw-rp-2-Node3.pdf}
\caption{Cumulative reward of node agent $N_3$ with different sizes of replay buffer}
\label{fig:reply-buff-N3}
\end{subfigure}
\hfil
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{./figures/ep-vs-rw-nonstationry-Node3.pdf}
\caption{Cumulative reward of node agent $N_3$ when trained with different number of agents}
\label{fig:nonstationary-N3}
\end{subfigure}
\hfil
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{./figures/Node3-delay-cdf.pdf}
\caption{CDF of delays of node agent $N_3$}
\label{fig:delay-cdf-N3}
\end{subfigure}

\caption{Demonstration of non-stationarity, effect of replay buffer size and delay measurements during training} %{\abde change data rates to Interest rates. Also, are we plotting the averages? Would be great if we can add the std to the plots}}
\label{fig:rep-buff-non-stationarity}
\end{figure*}
%-------------------------
We show that the absence of replay buffer leads to higher oscillation which makes the system more susceptible to variations in the input states resulting in issues in convergence across all agents in the network. Deploying a replay buffer (we have tested different buffer sizes) often exhibits less variations, however, at the same time the cumulative reward does not move toward higher values as training progresses through every episode. This results in additional delays in reacting to any sudden change in the network characteristic (\eg input state, reward). As a result, experience replay is difficult to tune in such autonomous multi-agent RL scenario.
%}
%{\abde \textbf{PLEASE REVIEW WHAT I WROTE HERE}. Note: The goal is to support the message that we sell and we conclude with a sentence to support the challenge/issue. I hope we can do the same for every example}
%--------------------------------
% Even though $N_3$ achieved high cumulative reward with zero buffer size, the cumulative reward does not move toward higher values as training progresses through every episode.}

%===============================
% \textcolor{blue}{The main challenge of using replay buffer in a multi-agent scenario is to determine its size for the DQN of each agent. %{\abde Are we referring to Fig 5?} 
% In our packet forwarding problem, the replay buffer size may need to be varied for each node agent depending on the network topology, request rate, number of forwarding decisions etc. To provide an example using the topology in Figure~\ref{fig:topo-Sprint-2}, let us assume that the replay buffer of each node agent is set to 300 experience tuples. With 300 interest rate from the consumer and $N_3$ distributing interests to $N_6$ and $N_9$, the buffer of $N_6$ will contain more diverse state transition data compared to $N_9$. Because unlike $N_3$, $N_6$ will make less number of forwarding decisions per second and will fill the buffer slowly. As a result, the buffer will contain experience tuples from various policies. Consequently, some of the experience tuples produced by a bad policy such as forwarding interests to $N_5$ or $N_{10}$ is likely to be sampled and diverge the training of agent $N_6$ from the optimal policy which can be the decision to forwarding interests to $N_4$.}

%------------------------------
% multiple parameters 
% For the topology in Figure~\ref{fig:topo-Sprint-2}, we conducted a set of probing experiments to determine the optimal values of episode duration and number of episodes. }
%--------------------------
% The main challenge here is to determine the optimal duration of the simulation (episode) and the optimal number of episodes, for the most efficient training and generalization of the RL agents. %The requirement is to train the DQNs sufficiently without the possibility of overfitting.
% The optimal values of these parameters will be different based on the topology of the network and the network characteristics. 
% For the topology in Figure~\ref{fig:topo-Sprint-2}, we conducted a set of probing experiments to determine the optimal values of episode duration and number of episodes.
% %To demonstrate the impact of simulation duration we conducted a set of probing experiments in our Figure~\ref{fig:topo-Sprint-2} topology . 
% In Figure~\ref{fig:duration-N3}, we show the cumulative reward obtained by agent $N_3$ per episode when we train the agents for 50 episodes with different episode length. We found that with episode length of 60 seconds(s), agent $N_3$ achieves higher cumulative reward compared to that of other episode lengths. Even though we used 60~s episode length in all our experiments, from Figure~\ref{fig:duration-N3} we observe that the cumulative reward fails to improve as training progresses through each episode. Therefore, its quite challenging to find the optimum value of episode length, even when the topology and network characteristics are known.
%---------------------------------
%esult in the optimal generalization for our test network under varying network traffic. 

%{\abde I like that we mention that we use simulations to investigate this, but again the message that we sell here is that we are able to find an optimal. The message that we love to convey is that we failed to find an optimal (totally different). We were not able to find the optimal, because even BR can beat us.}

%\textbf{HAS BEEN REWRITTEN TO ADDRESS THE COMMENT}    
%------------------------------
\subsection{Non-stationarity of the Environment}

One of the major challenges for distributed autonomous multi-agent RL is the \emph{non-stationarity}. 
%The environment is non-stationary from the perspective of each agent, as other agents in the environment are independently learning, ruling out any convergence guarantees. 
In a multi-agent setting of Markov Decision Process, the state and reward of each agent depend on the actions of all agents and every agent adapts its behaviors in the context of other co-adapting learning agents.
Since all agents are learning concurrently, the environment is not stationary and constantly changing from the perspective of any given agent. This phenomenon actually rules out any convergence guarantees.
%--------------------------
%One of the major challenges for distributed multi-agent RL is the \emph{non-stationarity}, which implies that there is a gap between the environmental dynamics from which the agent has learned and the current dynamics in which it is learning.%~\cite{foerster2017stabilising}. 
%The environment is non-stationary from the perspective of each agent, as other agents in the environment are independently learning, ruling out any convergence guarantees. In this multi-agent setting of Markov Decision Process, the state and reward of each agent depend on the actions of all agents and every agent adapts its behaviors in the context of other co-adapting learning agents.
%%This means In the a multi-agent setting of Markov Decision Process, 
%In addition, a multi-agent setting of Markov Decision Process, the state and reward of each agent depend on the actions of all agents. Every agent adapts its behaviors in the context of other co-adapting learning agents. 
%Since all agents are learning concurrently, the environment is not stationary and constantly changing from the perspective of any given agent.
%--------------------------    
    % \textcolor{blue}{To better illustrate the challenge from the perspective of packet forwarding, we consider the topology in Figure~\ref{fig:topo-Sprint-2} where agents are installed at nodes $N_3$, $N_6$ and $N_9$. Let us assume that the choice of $N_9$ and $N_8$ as next hops for node agent $N_3$ and $N_9$ respectively yields the optimal performance (minimum overall delay) of the network. Consider a scenario where $N_3$ has already finished exploration and found that forwarding interests to the next hop node $N_9$ is the best policy for itself. On the other hand, $N_9$ has not finished probing the environment and is still exploring its actions of forwarding interests to its outgoing interfaces. In this scenario, $N_9$ is distributing the interests received from $N_3$ and will be forwarding some interests to $N_4$ which leads to a  longer-delay path to the producer. The RTTs of these interests will decrease the reward values and change states of $N_3$. 
    % %[{\abde This is not clear. When N3 converged, N9 was also distributing. What's the change here?}]. 
    % Since $N_3$ is still learning, it may change its policy and start forwarding interests to the other next hop $N_6$. 
    % %{abde [In your example N3 converged. What do you mean by still learning?]}. 
    % In the mean time, $N_9$ will learn that $N_8$ is the best next hop to forward interests. Now, $N_9$ may be receiving the interests sent by $N_3$ via $N_6$ and $N_{10}$. Using $N_8$ as the next hop for forwarding all interests received by $N_9$ will make the $N_9-N_8$ link congested resulting in higher delays. This event may cause $N_9$ to change its policy and use $N_4$ as the next hop. $N_3$ finds that forwarding to $N_6$ is generating lower reward values and changes its policy again to $N_9$. By this time $N_9$ has already changed its policy of forwarding interests from $N_9$ to $N_4$. In this scenario, the decision policy of $N_3$ keeps changing through time because of the change of policies of other agents. As a result, at any moment, the joint action choice of agents $N_3$ and $N_9$ is not $<N_9,N_8>$, which will eventually lead to sub-optimal performance of the network.  }
 %================================   
    %{\abde Still not easy to follow and not able to understand the WHY of this? If you can answer these questions then we will be able to explain it better: (i) when does this happen (if loops, mesh, cascade, etc.)? and (ii) what triggers this challenge (exploration, congestion, etc.)?}
    
    %{\abde This is a very confusing example (we are using no less than 6-8 nodes in explain this challenge). No one would be able to follow the logic here. If we are not able to find a simple example using the given topology, I suggest we make a new 3 or 4 node topology to explain the problem. Example must have some details that explain the timeline and the challenge like what I drafted in Figure~\ref{fig:my_label}. link to source \url{https://drive.google.com/file/d/1_3mjgUS1yVqdkf5cpwoFpMxk_Q1ppWDk/view?usp=sharing} }
%--------------------------------    
% To illustrate the effect of nonstationary behavior, in Figure~\ref{fig:my_label}, we assume that the joint action (face selection) $<2,5>$ of agents $A_1$ and $A_3$ yields the optimal performance (minimum overall delay) of the network. Suppose at time $t_0$, agent $A_1$ is using face 2 and agent $A_3$ is using face 3. Now at time $t_1$, $A_1$ changed its face selection to 1, $A_3$ changed face to 5, and $A_2$ is using face 3. Then at time $t_2$, agent $A_3$ changed its policy to face 3, $A_1$ modified its policy to use face 2, and $A_2$ started using face 4. At all the time steps, agents are changing their actions based on the behavior of other agents. As a result, the optimal policy \ie the selection of face 2 and 5 by agents $A_1$ and $A_3$ respectively is not obtained. {\abde The figure I drew is a draft example, I think we need to list the correct times and interface or even change the topology a bit. }  
    
%----------Figure-5-----------------
%---------------------------
%   \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.90\linewidth]{ep-vs-rw-nonstationry-Node3}
%   \caption{Cumulative reward of node agent $N_3$ when training was done with one agent and two agents  
%   }
%   \label{fig:nonstationary-N3}
%   \end{figure}
%--------------------------
To demonstrate the effect of non-stationarity we performed two experiments on topology in Figure~\ref{fig:topo-Sprint-2}. %In one experiment, we train with only one agent in $N_3$ where its actions does not depend on any other node. In another experiment, we train with two agents: $N_3$ and $N_9$ where the actions of $N_3$ depend on the actions of $N_9$. We assume that in both cases all the other nodes without any agents know the forwarding next hop node to get optimal performance.
%----------------------
In one experiment, we put an agent only in node $N_3$ and train the single agent which will learn to choose between interfaces to node $N_6$ and $N_9$. In another experiment, we put agents in both $N_3$ and $N_9$ and train the two agents concurrently. Here, $N_9$ will learn to select between its next hops $N_8$ and $N_4$. We assume that in both cases all the other nodes without any agents know the forwarding next hop node to get optimal performance. 
In Figure~\ref{fig:nonstationary-N3}, we show the cumulative reward of node agent $N_3$ for the two cases. From Figure~\ref{fig:nonstationary-N3}, we observe that training with two agents cause the cumulative rewards of $N_3$ to be less and to fluctuate more compared to that of $N_3$ when training was done with one agent. %This is because with two agents $N_3$ will keep changing its policy based on the actions taken by $N_9$.
This is because with two agents the input state and reward of agent $N_3$ depends on the actions (face selections) of agent $N_9$. Similarly, the input state of agent $N_9$ is conditioned upon $N_3$'s  distribution of interests to $N_9$. As a result, during learning both agents keep changing their policy of choosing an interface based on the actions taken by each other. These actions can be conflicting (as shown by the large oscillations in the two agent cumulative reward) and result in degradation of performance as shown in our previous results. On the other hand, with only one agent $N_3$, its state and rewards solely depend on its actions, resulting in faster convergence and better performance. This phenomenon is amplified when: (i)  all agents are running simultaneously, (ii) the number of agents in the network scales, (iii) the network experience multiple concurrent flows (\eg many consumers and producers). 
One of the ways to deal with non-stationarity is to adopt a centralized architecture where agents will know the actions of one another. However, it is infeasible for forwarding packets in large distributed computer networks.

%---------------------
%{\abde Note: Review the last three sentences as I edited them.}   

%{\abde This example is better. Good.}}      
    
%\textcolor{blue}{The non-stationarity can be dealt by message passing among the agents with their current states. However, this will require a SDN type centralized server that can coordinate among all the individual agents. This will be contrasting to the principle of stateful forwarding, which aims to make local forwarding decisions. Therefore this challenge persists in the IQL based forwarding strategy and is one of the reasons for the moderate performance of IDQF.} 
    
\subsection{Partial Observability of the Environment}
Another key factor in autonomous multi-agent RL is the \emph{partial observability}. In many real-world environments, agents cannot perceive the complete state of the environment. For example, in our context of packet forwarding, the agents at each router observe the state per interface per producer in terms of some parameters such as RTT or drop ratio which indicate the congestion status of their respective interfaces. However, agents cannot distinguish certain events, which may occur beyond their local knowledge, including if two or more of their available interfaces lead to overlapping paths towards a given producer, or if a given interface will compete with other distant flows (\ie using portions of the path towards the producer). All these situations may result in similar measured rewards, but require different mitigation (\eg drop packets, choose different interface, etc.). Besides, the node agents neither know the actions (next hop choices) other agents have taken nor can compute the global reward (overall delay in consumer) by themselves. In order to find a globally optimal policy, the agents need to take into account the states and behavior of other agents and adapt to the joint behavior accordingly. Global observability, such as in SDN, or message-exchange-based coordination is needed to overcome this problem. We argue that even message-exchange-based coordination is challenging due to delays in message exchanged across agents unless a mechanism such as separate control channel is in place  to transmit the messages out of band. %We discuss this challenge in the next subsection.
    
    %{\abde Don't see how the partial observability creates challenges. Does it lead to non-convergence? Or does it converge to non-optimal values. These are two different things, and I still think that these cannot be merged. You know better, so please explain.}
    
    % \begin{figure}
    %     \centering
    %     \includegraphics{figures/stationarity.pdf}
    %     \caption{Caption}
    %     \label{fig:my_label}
    % \end{figure}
    %-------------------------
%==============================
%\textcolor{red}{REMOVE N3-delay CDF from title and rename Y-axis label to CDF. REPLACE Q-learning citation with IQL citation}
%---------------------------------    
%\subsection{Unavailability of Instantaneous Reward}
\subsection{Inability to Assess Actual Reward}
Most of the RL algorithms have been designed for environments where the feedback or reward is instantly available upon execution of an action. These algorithms cannot adequately solve the problems where actual rewards can not be assessed or are not  available immediately~\cite{shen2016reinforcement}. The delayed feedback phenomenon is also visible in our packet forwarding problem.
In any network, delays occur due to many factors including transmission, propagation, queuing, etc. Thus, measuring the state parameters and true reward value for the last action can not be collected before the next decision step occurs. Since RTTs could take from few milliseconds to seconds (especially due to drop and re-transmissions), estimating the current state and reward, \eg RTT or drops, for any forwarded Interest packet is pushed by additional and often variable delays. Throughout these waiting times, the agents will have to make forwarding decisions for incoming Interest packets and assign some approximated rewards against its state-action observations. These approximated rewards make it difficult to determine which of the state-action pairs contributed to the achievement of the optimization goal. This can lead to agents obtaining sub-optimal policies. 
%---------------------------
% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.90\linewidth]{Rt200-net-delay-cdf}
% \caption{CDF of delays when consumers request rate is 200 interests/sec.  
%   }
% \label{fig:net-delay-cdf}
% \end{figure}
%-----------------------
%For example, the topology in Figure~\ref{fig:topo-Sprint-2} shows that the theoretical RTT of the optimal path between the consumer and the producer is 53ms. However, based on our experiments we measured delays ranging from 79ms (\ie counting queuing and other processing delays) to 1s (maximum delay before dropping PIT entries), where more than 70\% of the delay measurements exceeded 500ms.
For example, the topology in Figure~\ref{fig:topo-Sprint-2} shows that the theoretical RTT of the optimal path between router $N_3$ and the producer is 49.51ms.
However, as shown in Figure~\ref{fig:delay-cdf-N3}, based on our experiments we measured delays ranging from 61ms (\ie counting queuing and other processing delays) to 1s (maximum delay before dropping PIT entries), where more than 50\% of the delay measurements exceeded 300ms. 
These large variations in the delay measurements in a controlled experiment, where number of flows, traffic, and routes are static, pushes autonomous multi-agent RL approaches to make approximate forwarding decisions which are often far from the optimal policy. 



%show that the , we deduce that the RTT of a single  Interest sent from $N_3$ through  minimum  delay  path should be around 41 ms. However, in our experiments, we observe that the RTTs vary starting from 61 ms and goes up-to 1.4 s with a mean of 400 ms.
%{\abde Why are we measuring starting from N3. our plots are end-to-end (consumer-producer), correct? Upload one of the CDF figures and I will edit this part. We can add more info here.} 
%----------------------------


%To illustrate this challenge, we provide an example considering the topology in Figure~\ref{fig:topo-Sprint-2}. Let us assume that the consumer, $C_0$ is requesting data at a rate of 300 interests/sec. That means, every 10 milliseconds (ms) $N_3$ will receive 30 interests from the consumer. Suppose all node agents make forwarding decisions every 10 ms. So if $N_3$ chose $N_9$ as next hop at last decision time step, it will forward 30 interest packets to $N_9$. Ignoring any queuing delay and packet processing delay in the routers, from Figure~\ref{fig:topo-Sprint-2}, we can deduce that the RTT of a single Interest sent from $N_3$ through minimum delay path $N_9-N_8$ is 41.44 ms.  Therefore, the RTT of 30 packets will be 1.24 s. {\abde \textbf{That's not correct! this assumes that they will be sent sequentially}! I think we don't need an example for this challenge or I can draft one easy example.} This implies that the true reward value of the action (selecting interface) that $N_3$ took should be 1.24 s. However, by this time $N_3$ will have to make more than 10 forwarding decisions. That means, $N_3$ has to assign to its previous action an approximated reward value \eg  the average RTT of the Data packets received between last decision step and current decision step.   

%================================
% \subsection{Non-stationarity of the Environment}

%     \textcolor{blue}{One of the major challenges for distributed multi-agent RL is the \emph{non-stationarity}, which imply that there is a gap between the environmental dynamics from which the agent has learned and the current dynamics in which it is learning~\cite{foerster2017stabilising}. The environment is nonstationary from the perspective of each agent, as other agents in the environment are independently learning, ruling out any convergence guarantees. In this multi-agent setting of Markov Decision Process, the state and reward of each agent depend on the actions of all agents and every agent adapts its behaviors in the context of other co-adapting learning agents.
%     %This means In the a multi-agent setting of Markov Decision Process, 
%     %In addition, a multi-agent setting of Markov Decision Process, the state and reward of each agent depend on the actions of all agents. Every agent adapts its behaviors in the context of other co-adapting learning agents. 
%     Since all agents are learning concurrently, the environment is not stationary and constantly changing from the perspective of any given agent. }
    
%     \textcolor{blue}{To better illustrate the challenge from the perspective of packet forwarding, we consider the topology in Figure~\ref{fig:topo-Sprint-2} where agents are installed at nodes $N_3$, $N_6$ and $N_9$. Let us assume that the choice of $N_9$ and $N_8$ as next hops for node agent $N_3$ and $N_9$ respectively yields the optimal performance (minimum overall delay) of the network. Consider a scenario where $N_3$ has already finished exploration and found that forwarding interests to the next hop node $N_9$ is the best policy for itself. On the other hand, $N_9$ has not finished probing the environment and is still exploring its actions of forwarding interests to its outgoing interfaces. In this scenario, $N_9$ is distributing the interests received from $N_3$ and will be forwarding some interests to $N_4$ which leads to a  longer-delay path to the producer. The RTTs of these interests will decrease the reward values and change states of $N_3$ [{\abde This is not clear. When N3 converged, N9 was also distributing. What's the change here?}]. Since $N_3$ is still learning, it may change its policy and start forwarding interests to the other next hop $N_6$ {abde [In your example N3 converged. What do you mean by still learning?]}. In the mean time, $N_9$ will learn that $N_8$ is the best next hop to forward interests. Now, $N_9$ may be receiving the interests sent by $N_3$ via $N_6$ and $N_{10}$. Using $N_8$ as the next hop for forwarding all interests received by $N_9$ will make the $N_9-N_8$ link congested resulting in higher delays. This event may cause $N_9$ to change its policy and use $N_4$ as the next hop. $N_3$ finds that forwarding to $N_6$ is generating lower reward values and changes its policy again to $N_9$. By this time $N_9$ has already changed its policy of forwarding interests from $N_9$ to $N_4$. In this scenario, the decision policy of $N_3$ keeps changing through time because of the change of policies of other agents. As a result, at any moment, the joint action choice of agents $N_3$ and $N_9$ is not $<N_9,N_8>$, which will eventually lead to sub-optimal performance of the network.  }
%     {\abde This is a very confusing example (we are using no less than 6-8 nodes in explain this challenge). No one would be able to follow the logic here. If we are not able to find a simple example using the given topology, I suggest we make a new 3 or 4 node topology to explain the problem. Example must have some details that explain the timeline and the challenge like what I drafted in Figure~\ref{fig:my_label}. link to source \url{https://drive.google.com/file/d/1_3mjgUS1yVqdkf5cpwoFpMxk_Q1ppWDk/view?usp=sharing} }
    
% \subsection{Partial observability of the environment}
%     \textcolor{blue}{Another key factor in multi-agent RL is the \emph{partial observability}. In many real-world environments, agents can't perceive the complete state of the environment, instead get partial observations. For example, in our context of packet forwarding problem,
%     the agents at each router observe the state per interface per producer in terms of some parameters such as RTT which indicates the congestion status of their respective interfaces. However, this actually provides incomplete information because agents cannot figure out events beyond their local knowledge including if their available interfaces leading to a given producer are overlapping or no, or if they will compete with other flows using portions of the path towards the producer. All these events may result in similar measured rewards, but require different mitigation (\eg drop packets, choose different interface, etc.).
%     Besides, the node agents neither know the actions (next hop choices) other agents have taken nor can compute the global reward (overall delay in consumer) by themselves.
%     In order to find a globally optimal policy, the agents need to take into account the states and behavior of other agents and adapt to the joint behavior accordingly.} 
    
%     {\abde Don't see how the partial observability creates challenges. Does it lead to non-convergence? Or does it converge to non-optimal values. These are two different things, and I still think that these cannot be merged. You know better, so please explain.}
    
%     \begin{figure}
%         \centering
%         \includegraphics{figures/stationarity.pdf}
%         \caption{Caption}
%         \label{fig:my_label}
%     \end{figure}
%     %-------------------------
    %Since each agent has their own independent observation-action and depends on the decision policies of the other agents that are continuously updated in the learning process, consequentially there would be variation in the expected reward for a state-action pair of a given agent. If this variation is not taken into account this would result in inaccurate estimated reward for state-action pairs and therefore good policies at a given time point would change over time. %This variation violates the basic stationary assumption for establishing the convergence of DQN algorithm. 

    %-------------------------
    %In most of the real-world environments, it is impossible for an agent to perceive the complete state of the environment and take appropriate actions to maximize the global reward. %gain access to the global reward. 
    %In our context of packet forwarding, % to optimize the network performance, 
    %the agents at each router observe the state per interface per producer in terms of some parameters such as RTT which indicates the congestion status of their respective interfaces. However, this actually provides incomplete information because agents cannot figure out events beyond their local knowledge including if their available interfaces leading to a given producer are overlapping or no, or if they will compete with other flows using portions of the path towards the producer. All these events may result in similar measured rewards, but require different mitigation (\eg drop packets, choose different interface, etc.). If partial observation of the agents is treated as the whole state of the network environment, the DQN will have difficulty converging and the agents may eventually learn sub-optimal solutions. 
%-----------------------------
   %\item \textbf{Non-stationary target in real-time deployment:} 
    %\item \textbf{Non-stationarity and Convergence} 
    %\textcolor{blue}{Unlike supervised learning, the ground truth labels (target) to the deep neural network (DNN) of reinforcement learning known as DQN are not fixed and needs to be calculated. DNN will usually converge towards the desired target values after certain number of iterations when these values are fixed, but will have problem converging when the target also moves. The target values in RL algorithm will change during learning since those are approximated using the weights of DNN itself and the weights are always changing after each decision epoch. As a solution to the convergence problem of DNN, a second DNN called target DQN with same structure as the original DQN is widely used. Instead of computing the target values using the current parameters of the original DQN, it is computed with target DQN. The target DQN is then infrequently updated with the learned weights of the original DQN. In a multi-episode RL training algorithm, target DQN can be easily applied by allowing it to  update its parameters from the original DQN after each episode ends. With this setting, the training behaves more like a supervised learning and make the learning stable. }
    
    % When an agent is deployed in a network environment, it is expected that the agent will also learn while taking actions based on the learned policy from its training.
    % However, in deployment mode there is no concept of episode for the agent like training mode. So we can't use the target DQN for the agent. Even if we use a target DQN, how frequently to update its parameters becomes a significant problem. Due to the absence of target DQN, target values will depend on original DQN itself and will be chasing a moving target while learning in deployment mode. Since the targets can't move closer to any ground truth, the learning process of DQN destabilizes in deployment mode. 
    
    %\item \textbf{Non-stationary environment:}
    % One of the key challenges for distributed multi-agent RL is the \emph{non-stationarity}~\cite{foerster2017stabilising}. Every agent adapts its behaviors in the context of other co-adapting learning agents. Since all agents are learning concurrently, the environment is constantly changing from the perspective of any given agent. In order to find a globally optimal policy, the agents need to take into account the behavior of other agents and adapt to the joint behavior accordingly. Since each agent has their own independent observation-action and depends on the decision policies of the other agents that are continuously updated in the learning process, consequentially there would be variation in the expected reward for a state-action pair of a given agent. If this variation is not taken into account this would result in inaccurate estimated reward for state-action pairs and therefore good policies at a given time point would change over time. This variation violates the basic stationary assumption for establishing the convergence of DQN algorithm. 
%---------------------------
    %It becomes harder when DNN is used as Q-function approximator. %To provide an example of non-stationary property in networking environment, let us 
%---------Example-------------
    %To better illustrate the challenge from the perspective of packet forwarding, we consider the topology in Figure~\ref{fig:topo-Sprint-2} where agents are installed at nodes $N_3$ and $N_9$. One of the outgoing interfaces of $N_3$ is connected to $N_9$, and $N_9$ is connected to other nodes. Let us assume that $N_3$ has already finished exploration during the training and found that to forward interests to the next hop node $N_9$ is the \emph{best policy}. On the other hand, $N_9$ has not finished probing the environment and is still exploring its actions of forwarding interests to its outgoing interfaces. In this scenario, the decision policy of $N_3$ will get effected because it is still learning from the state and rewards attached to the interface to $N_9$. That means, the learning process of $N_3$ depends on the actions node $N_9$ takes. It is likely that the best policy that $N_3$ has learned previously, could alter after some time because of the actions taken by $N_9$. {\abde The example is not clear. Are you suggesting that N3 has prematurely selected N9 while it could have selected N6? Let us be specific with hypothetical assumptions (but use short sentences).}
%----------------------------    
    %\textcolor{blue}{Unlike supervised learning, the ground truth labels (target) to the deep neural network (DNN) of reinforcement learning known as DQN are not fixed and needs to be calculated. 
%------example-2--------------
%In this scenario, the decision policy of $N_3$ will get effected because it is still learning from the state and rewards attached to the interface to $N_9$. That means, the learning process of $N_3$ depends on the actions node $N_9$ takes. It is likely that the best policy that $N_3$ has learned previously, could alter after some time because of the actions taken by $N_9$. {\abde The example is not clear. Are you suggesting that N3 has prematurely selected N9 while it could have selected N6? Let us be specific with hypothetical assumptions (but use short sentences).}

%=====================  
%\subsection{Partial Observability}
% In most of the real-world environments, it is impossible for an agent to perceive the complete state of the environment and take appropriate actions to maximize the global reward. %gain access to the global reward. 
% In our context of packet forwarding, % to optimize the network performance, 
% the agents at each router observe the state per interface per producer in terms of some parameters such as RTT which indicates the congestion status of their respective interfaces. However, this actually provides incomplete information because agents cannot figure out events beyond their local knowledge including if their available interfaces leading to a given producer are overlapping or no, or if they will compete with other flows using portions of the path towards the producer. All these events may result in similar measured rewards, but require different mitigation (\eg drop packets, choose different interface, etc.). If partial observation of the agents is treated as the whole state of the network environment, the DQN will have difficulty converging and the agents may eventually learn sub-optimal solutions. 
    
% Moreover, the total reward will also depend on the joint actions of all the agents. The agents neither know the actions other agents have taken nor can compute the global reward by themselves. For example, let us assume that the choice of $N_9$ as next hop for node agent $N_3$ and the choice of $N_8$ as next hop for node agent $N_9$ is the optimal solution. Given the local observations, agent $N_3$ may learn that choosing $N_6$ next hop is optimal, whereas $N_9$ may learn that choosing $N_8$ next hop is optimal. However, their joint action choice $<N_6, N_8>$ actually results in a sub-optimal solution.   

%=========================
% \subsection{DQN Convergence}
% Another problem in multi-agent RL algorithm is the convergence of the agents' DQNs. 
% The DQN usually converges towards the desired target values after certain number of iterations when the target values or the ground truths are fixed but the convergence is challenging when there are moving targets.  
% The target values in DQN algorithm will change during learning since those are approximated using the weights of DQN itself and the weights are always changing after each decision step. As a solution to the convergence problem of DQN, a second neural network called target DQN with same structure as the original DQN is widely used. Instead of computing the target values using the current parameters of the original DQN, it is computed with target DQN. The target DQN is then infrequently updated with the learned weights of the original DQN. In a multi-episode DQN training algorithm, target DQN can be easily applied by allowing it to  update its parameters from the original DQN after each episode ends. With this setting, the training behaves more like a supervised learning and makes the learning relatively stable. 
% %This stationary assumption is also called Markov property, which implies that the reward and current state of an individual agent will depend only on the previous state and action taken.
% However, when an agent is deployed in a network environment, it is expected that the agent will also learn while taking actions based on the learned policy from its training. However, in deployment mode there is no concept of episode for the agent like training mode. So we can't use the target DQN for the agent. Even if we use a target DQN, how frequently to update its parameters becomes a significant problem. Due to the absence of target DQN, target values will depend on original DQN itself and will be chasing a moving target while learning in deployment mode. Since the targets can't move closer to any ground truth, the learning process of DQN may destabilize in the deployment mode. 
%--------------------------   
%============NEW==================
%==========Convergence============
% \subsection{Convergence Enhancement}
% \textcolor{blue}{To aid the convergence of DQN and enhance its generalizing ability%and minimize the chances of divergence 
% two techniques namely \emph{target DQN} and \emph{experience replay} are generally preferred~\cite{mnih2015human}. The challenges of using these techniques in %multi-agent setting such as 
% our packet forwarding problem in network are described in the following subsections.}
%----------Target DQN--------------
% \subsubsection{Target DQN}
% \textcolor{blue}{The DQN usually converges towards the desired target values after certain number of iterations when the target values or the ground truths are fixed, but the convergence is not guaranteed when there are moving targets. The target values in DQN will change during learning since those are approximated using the weights of same DQN itself and the weights are always changing after each decision step. To solve this issue, a second neural network called \emph{target DQN} with same structure as the original DQN is used. Instead of computing the target values using the current weights of the original DQN, it is computed with target DQN. The target DQN is then infrequently updated (usually after certain number of decision steps) with the learned weights of the original DQN. With this setting, the training behaves more like a supervised learning and makes the learning relatively stable. }

% \textcolor{blue}{ One of the main challenges of using target DQN is to determine the temporal gap to update its weights with those of original DQN, specially in a multi-agent setting similar to our packet forwarding problem where each router is equipped with two DQNs. The weight update frequency may need to be varied for each agent depending on the request rate of the consumer, number of interest packets received by a router etc. % distance from consumer and producer
% For example, let us assume that in Figure~\ref{fig:topo-Sprint-2} the consumer, $C_0$ is requesting 300 interests per second and all node agents are making forwarding decisions every 10 milliseconds. That means, in every 1 second $N_3$ will make approximately 100 forwarding decisions. If we assume that $N_3$ is distributing the interests between $N_6$ and $N_9$, then $N_6$ and $N_9$ will not make the same number of forwarding decisions as $N_3$ does in 1 second. In this case, setting the update frequency to be a fixed number of decision step for $N_3, N_6,$ and $N_9$ will not be appropriate and may effect the learning process.   
% Another problem of applying target DQN in a multi-agent network scenario is that it includes additional memory requirements and computational complexity for each router.   }
%================================
%\textcolor{blue}{The main challenge of using replay buffer in a multi-agent scenario is to determine its size for the DQN of each agent. In the context of our packet forwarding problem, the replay buffer size will depend on the interest rate and may need to be varied for each node agent. For example, suppose all node agents in Figure~\ref{fig:topo-Sprint-2}} topology make forwarding decisions ever
%However, when an agent is deployed in a network environment, it is expected that the agent will also learn while taking actions based on the learned policy from its training. However, in deployment mode there is no concept of episode for the agent like training mode. So we can't use the target DQN for the agent. Even if we use a target DQN, how frequently to update its parameters becomes a significant problem. Due to the absence of target DQN, target values will depend on original DQN itself and will be chasing a moving target while learning in deployment mode. Since the targets can't move closer to any ground truth, the learning process of DQN may destabilize in the deployment mode. 

%---------------------------------
    %\todo[inline]{This is true. But can we say that if these agents will take turns, RL could converge (or do better)? We must discuss solutions in this paper. Taking terns can be easily implemented here.}
    
    %\item \textbf{Catastrophic Forgetting and Generalization}: %in real-time deployment}:
%------------------------------ 
%=========Replay buffer=============
% \subsubsection{Size of replay buffer}
% \textcolor{blue}{
% During learning, instead of utilizing experience data (\ie state transition record as tuple $<$state, action, reward, next state$>$) for training immediately, the agent collects and stores the records in a circular memory buffer called \emph{experience replay} and update the weights of the DQN by randomly sampling mini-batches from it. The \emph{experience replay} technique helps the DQN to break correlation in observation sequences and learn from more independently and identically distributed past experience~\cite{mnih2015human} to stabilise the training. 
% The size of the \emph{experience replay} memory can influence the quality of learning of the resulting agent. %may cause bias in the function approximation estimate
% If the size of the \emph{experience replay} is large, then sometimes the recently experienced transitions will only be used for learning hundreds of steps later. Meanwhile, very old transitions, generated using an initially bad policy, can be used to train the network~\cite{zhang2017deeper}. 
% To demonstrate the effect of replay buffer size, we train IDQF with different sizes of replay memory. We show the cumulative reward obtained by node agent $N_3$ per episode of training in Figure~\ref{fig:reply-buff-N3}. We find that the cumulative reward obtained by $N_3$ varies with replay buffer size. Even though $N_3$ achieved high cumulative reward with no buffer size, the cumulative reward does to move toward higher values (convergence) as training progresses through every episode. }

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.90\linewidth]{ep-vs-rw-rp-2-Node3}
%   \caption{Cumulative reward of node agent $N_3$ with different sizes of replay buffer  
%   }
%   \label{fig:reply-buff-N3}
% \end{figure}

% \textcolor{blue}{The main challenge of using replay buffer in a multi-agent scenario is to determine its size for the DQN of each agent. %{\abde Are we referring to Fig 5?} 
% In our packet forwarding problem, the replay buffer size may need to be varied for each node agent depending on the network topology, request rate, number of forwarding decisions etc. To provide an example using the topology in Figure~\ref{fig:topo-Sprint-2}, let us assume that the replay buffer of each node agent is set to 300 experience tuples. With 300 interest rate from the consumer and $N_3$ distributing interests to $N_6$ and $N_9$, the buffer of $N_6$ will contain more diverse state transition data compared to $N_9$. Because unlike $N_3$, $N_6$ will make less number of forwarding decisions per second and will fill the buffer slowly. As a result, the buffer will contain experience tuples from various policies. Consequently, some of the experience tuples produced by a bad policy such as forwarding interests to $N_5$ or $N_{10}$ is likely to be sampled and diverge the training of agent $N_6$ from the optimal policy which can be the decision to forwarding interests to $N_4$.}
%==================================
%To demonstrate the effect of replay buffer, we ran IDQF with and without replay memory. We show the throughput of each experiment in Figure~\ref{fig:Model-comp-throughput}. From Figure~\ref{fig:Model-comp-throughput}, we observe that when replay memory is used for agents, the total throughput is around 12\% better than the total throughput achieved by agents without replay memory in their DQN. When no replay memory is used, the DQN updates its weights for every training sample and changes its predictions frequently resulting in high variance in the throughput. However, when agents have replay memory, the DQN samples training data from that memory and updates the weights as a mini-batch. This causes the throughput to be high and more stable.
%-----------------------------------
% \subsection{Catastrophic Forgetting}
% One of the challenges of DQN is that the weights of the neural networks are updated regularly and the new learning may unintentionally erase a part of the previously acquired knowledge in a non-stationary environment. This is also referred to as catastrophic forgetting~\cite{kaplanis2018continual}.
% We used the concept of replay memory to avoid catastrophic forgetting.
% During learning, instead of utilizing state transition samples($<$state, action, reward, next state$>$) as training data immediately, the agent collects and stores the samples in a circular memory buffer called \emph{experience replay} and update the weights of the DQN by randomly sampling mini-batches from it. The \emph{experience replay} technique helps the DQN to break correlation in observation sequences and learn from more independently and identically distributed past experience~\cite{mnih2015human}. 

% The size of the \emph{experience replay} memory can heavily influence the quality of learning of the resulting agent. If the size of the \emph{experience replay} is large, then sometimes the recently experienced transitions will only be used for learning hundreds of steps later. Meanwhile, very old transitions, generated using an initially bad policy, can be used to train the network~\cite{zhang2017deeper}. To summarize, although the replay memory can minimize catastrophic forgetting, it can not completely prevent forgetting and pose as a challenge.
%-----------------------
% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.90\linewidth]{Model-comp-throughput}
%   \caption{Throughput comparison with different settings of IDQF: agents with replay buffer and without replay buffer  
%   }
%   \label{fig:Model-comp-throughput}
% \end{figure}
%-----------------------
%To demonstrate the effect of replay buffer, we ran IDQF with and without replay memory. We show the throughput of each experiment in Figure~\ref{fig:Model-comp-throughput}. From Figure~\ref{fig:Model-comp-throughput}, we observe that when replay memory is used for agents, the total throughput is around 12\% better than the total throughput achieved by agents without replay memory in their DQN. When no replay memory is used, the DQN updates its weights for every training sample and changes its predictions frequently resulting in high variance in the throughput. However, when agents have replay memory, the DQN samples training data from that memory and updates the weights as a mini-batch. This causes the throughput to be high and more stable.
%==============================
%----------------------
%Today’s deep learning methods struggle to learn rapidly in the incremental, online settings that are most natural for the reinforcement learning algorithms. The problem is sometimes described as one of `catastrophic interference' or `correlated data.' When something new is learned it tends to replace what has previously been learned rather than adding to it, with the result that the benefit of the older learning is lost. Techniques such as “replay buffers” are often used to retain and replay old data so that its benefits are not permanently lost.
    
    %--------------------
    % The size of the \emph{experience replay} memory can heavily influence the quality of learning of the resulting agent.}
    % If the size of the \emph{experience replay} is large, then sometimes the recently experienced transitions will only be used for learning hundreds of steps later. Meanwhile, very old transitions, generated using an initially bad policy, can be used to train the network~\cite{zhang2017deeper}. Although the replay memory can minimize catastrophic forgetting, it can not completely prevent forgetting.
   
%   We run experiments to highlight the effect of catastrophic forgetting by comparing two schemes, with and without replay memory during training (Figure~\ref{fig:ep-vs-rw}). We plot the average reward in every episode for node agent $N_3$ in our topology. From Figure~\ref{fig:ep-vs-rw}, we observe that when no replay memory is used, the average reward of $N_3$ oscillates too much compared to the average reward when replay memory is used. When no replay memory is used, the DQN updates its weights for every training sample and changes its predictions frequently resulting in high variance in the average reward. However, when agents have replay memory, the DQN samples training data from that memory and updates the weights. This causes the average reward of each agent to vary slowly.  {\abde Is the main message here, replay memory is best? If that is the case then why we list this as a challenge? If it is costly to do so then we need to talk about it here (how costly?)}      
   

%============================  
%In addition, the exhaustiveness of the sample set and the method of training play a significant role in proper generalization of the DNN. In our problem, the goal of every agent is to maximize its cumulative reward or the expected return. The expected return is simply the sum of all rewards the agent received starting from the initial state to a terminal state of the environment. An agent can reach a terminal state if certain score is obtained or the task is complete. The learning of a optimized policy works better if we know what return to expect and train the agents over and over again by resetting the state to the initial state and start new agent-environment interaction. In our case, we don't know a terminal state or a target score for the network environment. %So to make a final time step or terminal state we consider running a simulation for a specific period of time and call it a episode. 
%Therefore, we run the simulation for a specific period of time and consider it as an episode. The duration of the episode and the number of episodes play an important role in the generalization of the DNN. The requirement is to train the DNN model sufficiently without the possibility of over-fitting. This will be different for different network topology and network environment. We conducted a set of probing experiments and found that the episode length of $60~S$ and keeping the number of episodes as $50$, result in the optimal generalization for our test network under varying network traffic. 
%----------------------------
 %\textcolor{red}{@Abu: lets include an example case with different episode size and the generalization performance}

%  \begin{figure}[h!]
% %   \begin{subfigure}{0.6\columnwidth}
%  \centering
%  \includegraphics[width=0.8\linewidth]{./figures/ep-vs-rw-Node3.pdf}
%  %\caption{$N_3$}
%  \label{fig:ep-vs-rw-Node3}
% %  \end{subfigure}
% %  \begin{subfigure}{0.6\columnwidth}
% %  \centering
% %  \includegraphics[width=\linewidth]{./figures/ep-vs-rw-Node3.pdf}
% %  %\caption{$N_3$}
% %  \label{fig:ep-vs-rw-Node3}
% %  \end{subfigure}
% %  \begin{subfigure}{0.45\columnwidth}
% %  \centering
% %  \includegraphics[width=\linewidth]{./figures/ep-vs-rw-Node4.pdf}
% %  \caption{$N_4$}
% %  \label{fig:ep-vs-rw-Node4}
% %  \end{subfigure}
% %  \begin{subfigure}{0.45\columnwidth}
% %  \centering
% %  \includegraphics[width=\linewidth]{./figures/ep-vs-rw-Node6.pdf}
% %  \caption{$N_6$}
% %  \label{fig:ep-vs-rw-Node6}
% %  \end{subfigure}
% %  \begin{subfigure}{0.45\columnwidth}
% %  \centering
% %  \includegraphics[width=\linewidth]{./figures/ep-vs-rw-Node9.pdf}
% %  \caption{$N_9$}
% %  \label{fig:ep-vs-rw-Node9}
% %  \end{subfigure}
%  \caption{Average reward comparison between agents with replay buffer and without replay buffer for the agent at $N_3$}
%  \label{fig:ep-vs-rw}
%  \end{figure}
   
   
   %---------------------------
    %\todo[inline]{How is this different from the first challenge?}
    %   \item \textbf{Catastrophic forgetting:}
    %The new learning can abruptly erase the previously acquired knowledge. 
    
    %\todo[inline]{Still it is unclear to me what this means. Can we provide an example, say one node decides to forward on interface 1, why this action implies forgetting the past interfaces/states. I thought the model will always have weights and keep learning without forgetting. Please explain more. It is unclear to me so it can be unclear to reviewers.}
    
    %Although we used replay memory to avoid catastrophic forgetting, it can not be completely evaded. The exhaustiveness of the sample set and the method of training play a significant role in proper generalization of the DNN. \textcolor{red}{more on how we trained and why? Why did we train on the transient behaviour of the network? Why did we reset the simulator for each episode? Why didn't we run a continuous simulation for a long stretch of time?}
    
    % \textcolor{blue}{The goal of an agent in RL is to maximize its cumulative rewards which is also known as the expected return. The expected return is simply the sum of all rewards the agent received starting from the initial state to a terminal state of the environment. An agent can reach a terminal state if certain score is obtained or the task is complete. The learning of a optimized policy works better if we know what return to expect and train the agents over and over again by resetting the state to the initial state and start new agent-environment interaction. In our case, we don't know a terminal state or a target score for the network environment. So to make a final time step or terminal state we consider running a simulation for a specific period of time and call it a episode. }
    
    %\item  \textbf{Unavailability of instantaneous reward and Partial observability}  
 
    %-----------------------------
    %and nodes would need to wait until they timeout to detect such events. %Ideally the maximum value of the RTT can approach the PIT expiry time, which is defined as $2~S$ in our experimental set up. In addition, we must also wait for the PIT to expiry before we can label a interest packet as dropped. This implies that in most cases we will have to wait until the PIT expiry time threshold ($2~S$) for each agent to get the reward associated with a set of actions.
   
    %These finite duration lags in obtaining the reward makes learning difficult for agents at the routers 
    %({\abde can we say what kind of difficulty are we facing here. Does it take longer (or never) to converge? Does it add noise to the weights to the level that we can't recover from?}).
    
    %This delayed reward problem is prevalent in many real-world applications such as making decision to forward packets to the next hop for optimizing the network performance. 
    % For example, let us assume that the optimization goal of the network is to minimize the overall round-trip-time (RTT) delay of the packets. Thus, when a node agent forwards a packet, its reward signal should be the RTT delay of the packet. But in this case if the node agent needs to forward another packet before the RTT of the previous packet is available, then the agent is unable to map its previous decision to choose a next hop to the corresponding reward. Moreover, sometimes the reward can not be obtained at all if the packet drops at some node in the network before reaching the destination. This delay between taking an action and receiving the reward makes learning difficult for the node agents. 
    
    %\todo[inline]{If this is a well known problem, can we list one citation for describing the issue or better addressing it? I buy this challenge and can relate to it. I think we can use a small scenario to highlight the impact of this particular problem.}
    
    % \item \textbf{Catastrophic forgetting:}
    % The new learning can abruptly erase the previously acquired knowledge. \todo[inline]{Still it is unclear to me what this means. Can we provide an example, say one node decides to forward on interface 1, why this action implies forgetting the past interfaces/states. I thought the model will always have weights and keep learning without forgetting. Please explain more. It is unclear to me so it can be unclear to reviewers.}
    
    % Although we used replay memory to avoid catastrophic forgetting, it can not be completely evaded. The exhaustiveness of the sample set and the method of training play a significant role in proper generalization of the DNN. \textcolor{blue}{more on how we trained and why? Why did we train on the transient behaviour of the network? Why did we reset the simulator for each episode? Why didn't we run a continuous simulation for a long stretch of time?}
%---------------------------
% \subsection{DQN Training Method}
% \textcolor{blue}{The exhaustiveness of the sample training set and the method of training play a significant role in proper generalization of the DQN. In a multi-agent setting, the goal of every agent is to maximize its cumulative reward or the expected return. The expected return is simply the sum of all rewards the agent received starting from the initial state to a terminal state of the environment. An agent can reach a terminal state if certain score is obtained or the task is complete. The learning of an optimized policy works better if we know what return to expect and train the agents over and over again by resetting the state to the initial state and start new agent-environment interaction. The sequence of states, actions, and rewards starting from an initial state to a terminal state is known as episode. Thus the agents are iteratively trained through multiple episodes. In our case, we don't know a terminal state or a target score for the network environment. %So to make a final time step or terminal state we consider running a simulation for a specific period of time and call it a episode.
% Therefore, we run the network simulation for a specific period of time and consider it as an episode.
% After each simulation ends, the agents will gather a cumulative reward which is average RTT in our context. The goal of the agents is to maximize those rewards per simulation (episode) to reach an optimal policy.
% }
% %---------------------------
% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.90\linewidth]{ep-vs-rw-duration-Node3}
%   \caption{Cumulative reward of node agent $N_3$ when trained for different duration of simulation  
%   }
%   \label{fig:duration-N3}
% \end{figure}
% %--------------------------

% \textcolor{blue}{The main challenge here is to determine the duration of the simulation (episode) and the number of episodes for training the agents. The requirement is to train the DQNs sufficiently without the possibility of over-fitting. These two parameters will be different depending on the topology and network conditions. To demonstrate the impact of simulation duration we conducted a set of probing experiments in our Figure~\ref{fig:topo-Sprint-2} topology . In Figure~\ref{fig:duration-N3}, we show the cumulative reward obtained by agent $N_3$ per episode when we train the agents for 50 episodes with different episode length. We found that with episode length of 60 seconds(s), $N_3$ agent achieves higher cumulative reward compared to that of other episode lengths. Even though we used 60s episode length in all our experiments, from Figure~\ref{fig:duration-N3} we observe that the cumulative reward fails to improve as training progresses through each episode. }
% %esult in the optimal generalization for our test network under varying network traffic. 


% {\abde I like that we mention that we use simulations to investigate this, but again the message that we sell here is that we are able to find an optimal. The message that we love to convey is that we failed to find an optimal (totally different). We were not able to find the optimal, because even BR can beat us.}

% \textbf{HAS BEEN REWRITTEN TO ADDRESS THE COMMENT}    
    
%============================
    %\item \textbf{Partial observability:}
    %---------------------
    % \subsection{Partial Observability}
    % In most of the real-world environments, it is impossible for an agent to perceive the complete state of the environment and take appropriate actions to maximize the global reward. %gain access to the global reward. 
    % In our context of packet forwarding, % to optimize the network performance, 
    % the agents at each router observe the state per interface per producer in terms of some parameters such as RTT which indicates the congestion status of their respective interfaces. However, this actually provides incomplete information because agents cannot figure out events beyond their local knowledge including if their available interfaces leading to a given producer are overlapping or no, or if they will compete with other flows using portions of the path towards the producer. All these events may result in similar measured rewards, but require different mitigation (\eg drop packets, choose different interface, etc.). If partial observation of the agents is treated as the whole state of the network environment, the DQN will have difficulty converging and the agents may eventually learn sub-optimal solutions. 
    
    % Moreover, the total reward will also depend on the joint actions of all the agents. The agents neither know the actions other agents have taken nor can compute the global reward by themselves. For example, let us assume that the choice of $N_9$ as next hop for node agent $N_3$ and the choice of $N_8$ as next hop for node agent $N_9$ is the optimal solution. Given the local observations, agent $N_3$ may learn that choosing $N_6$ next hop is optimal, whereas $N_9$ may learn that choosing $N_8$ next hop is optimal. However, their joint action choice $<N_6, N_8>$ actually results in a sub-optimal solution.
%=============================
    %------------------------
   
    %Today’s deep learning methods struggle to learn rapidly in the incremental, online settings that are most natural for the reinforcement learning algorithms. The problem is sometimes described as one of `catastrophic interference' or `correlated data.' When something new is learned it tends to replace what has previously been learned rather than adding to it, with the result that the benefit of
    %the overall delay and maximize the throughput. 
    %    should minimize the RTT and/or maximize the throughput. However, the RTT can only be calculated once a packet is successfully delivered from a producer to a consumer. 
%============================= 

% \subsection{Non-stationarity of the Environment}

%     \textcolor{blue}{One of the major challenges for distributed multi-agent RL is the \emph{non-stationarity}, which imply that there is a gap between the environmental dynamics from which the agent has learned and the current dynamics in which it is learning~\cite{foerster2017stabilising}. The environment is nonstationary from the perspective of each agent, as other agents in the environment are independently learning, ruling out any convergence guarantees. In this multi-agent setting of Markov Decision Process, the state and reward of each agent depend on the actions of all agents and every agent adapts its behaviors in the context of other co-adapting learning agents.
%     %This means In the a multi-agent setting of Markov Decision Process, 
%     %In addition, a multi-agent setting of Markov Decision Process, the state and reward of each agent depend on the actions of all agents. Every agent adapts its behaviors in the context of other co-adapting learning agents. 
%     Since all agents are learning concurrently, the environment is not stationary and constantly changing from the perspective of any given agent. }
    
%     \textcolor{blue}{To better illustrate the challenge from the perspective of packet forwarding, we consider the topology in Figure~\ref{fig:topo-Sprint-2} where agents are installed at nodes $N_3$, $N_6$ and $N_9$. Let us assume that the choice of $N_9$ and $N_8$ as next hops for node agent $N_3$ and $N_9$ respectively yields the optimal performance (minimum overall delay) of the network. Consider a scenario where $N_3$ has already finished exploration and found that forwarding interests to the next hop node $N_9$ is the best policy for itself. On the other hand, $N_9$ has not finished probing the environment and is still exploring its actions of forwarding interests to its outgoing interfaces. In this scenario, $N_9$ is distributing the interests received from $N_3$ and will be forwarding some interests to $N_4$ which leads to a  longer-delay path to the producer. The RTTs of these interests will decrease the reward values and change states of $N_3$ [{\abde This is not clear. When N3 converged, N9 was also distributing. What's the change here?}]. Since $N_3$ is still learning, it may change its policy and start forwarding interests to the other next hop $N_6$ {abde [In your example N3 converged. What do you mean by still learning?]}. In the mean time, $N_9$ will learn that $N_8$ is the best next hop to forward interests. Now, $N_9$ may be receiving the interests sent by $N_3$ via $N_6$ and $N_{10}$. Using $N_8$ as the next hop for forwarding all interests received by $N_9$ will make the $N_9-N_8$ link congested resulting in higher delays. This event may cause $N_9$ to change its policy and use $N_4$ as the next hop. $N_3$ finds that forwarding to $N_6$ is generating lower reward values and changes its policy again to $N_9$. By this time $N_9$ has already changed its policy of forwarding interests from $N_9$ to $N_4$. In this scenario, the decision policy of $N_3$ keeps changing through time because of the change of policies of other agents. As a result, at any moment, the joint action choice of agents $N_3$ and $N_9$ is not $<N_9,N_8>$, which will eventually lead to sub-optimal performance of the network.  }
%     {\abde This is a very confusing example (we are using no less than 6-8 nodes in explain this challenge). No one would be able to follow the logic here. If we are not able to find a simple example using the given topology, I suggest we make a new 3 or 4 node topology to explain the problem. Example must have some details that explain the timeline and the challenge like what I drafted in Figure~\ref{fig:my_label}. link to source \url{https://drive.google.com/file/d/1_3mjgUS1yVqdkf5cpwoFpMxk_Q1ppWDk/view?usp=sharing} }
    
% \subsection{Partial observability of the environment}
%     \textcolor{blue}{Another key factor in multi-agent RL is the \emph{partial observability}. In many real-world environments, agents can't perceive the complete state of the environment, instead get partial observations. For example, in our context of packet forwarding problem,
%     the agents at each router observe the state per interface per producer in terms of some parameters such as RTT which indicates the congestion status of their respective interfaces. However, this actually provides incomplete information because agents cannot figure out events beyond their local knowledge including if their available interfaces leading to a given producer are overlapping or no, or if they will compete with other flows using portions of the path towards the producer. All these events may result in similar measured rewards, but require different mitigation (\eg drop packets, choose different interface, etc.).
%     Besides, the node agents neither know the actions (next hop choices) other agents have taken nor can compute the global reward (overall delay in consumer) by themselves.
%     In order to find a globally optimal policy, the agents need to take into account the states and behavior of other agents and adapt to the joint behavior accordingly.} 
    
%     %{\abde Don't see how the partial observability creates challenges. Does it lead to non-convergence? Or does it converge to non-optimal values. These are two different things, and I still think that these cannot be merged. You know better, so please explain.}
    
%     \begin{figure}
%         \centering
%         \includegraphics{figures/stationarity.pdf}
%         \caption{Caption}
%         \label{fig:my_label}
%     \end{figure}
%     %-------------------------
    
%     \subsection{Unavailability of Instantaneous Reward}
%     \textcolor{blue}{Most of the RL algorithms have been designed for environments where the feedback or reward is instantly available upon execution of an action. These algorithms can not adequately solve the problems where rewards are not immediately available~\cite{walsh2009learning}. The delayed feedback phenomenon is also visible in our packet forwarding problem.
%     In a network, depending on the topology and router configurations such as link propagation delays, queue size of routers, the actual measures of the next state parameters and true reward value for the last action can not be collected before the next decision step occurs. Because it could take from few milliseconds to seconds for the Data packet to arrive at the node agent after forwarding an Interest. Specially, when packets need to wait in the queue of intermediate routers for propagation, the delay of the Data packet increases. Moreover, packets may get dropped due to overflow of queue in a upstream router and the downstream routers do not have a definite way of knowing about this event. Thus computing the true RTT for an Interest packet becomes problematic. 
%     Throughout these waiting times, the agents will have to make forwarding decisions for incoming Interest packets and assign some approximated rewards against its state-action observations. These approximated rewards make it difficult to determine which of the state-action pairs contributed to the achievement of the optimization goal. This can lead to agents obtaining sub-optimal policies. }
    
%     \textcolor{blue}{To illustrate this challenge, we provide an example considering the topology in Figure~\ref{fig:topo-Sprint-2}. Let us assume that the consumer, $C_0$ is requesting data by 300 interest packets per second (s). That means, every 10 milliseconds (ms) $N_3$ will receive 30 interests from the consumer. Suppose all node agents make forwarding decisions every 10 ms. So if $N_3$ chose $N_9$ as next hop at last decision time step, it will forward 30 interest packets to $N_9$. Ignoring any queuing delay and packet processing delay in the routers, from Figure~\ref{fig:topo-Sprint-2}, we can deduce that the RTT of a single Interest sent from $N_3$ through minimum delay path $N_9-N_8$ is 41.44 ms.  Therefore, the RTT of 30 packets will be 1.24 s. This implies that the true reward value of the action (selecting interface) that $N_3$ took should be 1.24 s. However, by this time $N_3$ will have to make more than 10 forwarding decisions. That means, $N_3$ has to assign to its previous action an approximated reward value \eg  the average RTT of the Data packets received between last decision step and current decision step.   } 
    %It can lead to bad convergence properties of the DQN algorithm.
    %-------------------------
    %in this case the whole state of the network encompasses the states of all agents in the environment. 
    
    %which gives the cost of using an interface to reach a given producer.   which indicates the congestion status of an interface. %interface RTT and drop-rate. %Although the RTT and drop-rate are attributed with a set of interface available at a node, they may not reflect an exact status of the traffic at these interfaces 
    %------------------------
    %This is not totally true. We measure the state per interface per producer which gives the cost of using an interface to reach a given producer. Drops or delays in the paths are indications that the interface leads to congestion. There is no need to measure this per link.  
    %------------------------
    %This is due to the fact that the RTT and drop rates for an interface at a node are calculated for the total duration of interest initiation and packet delivery. 
    %------------------------
    %This means that a packet would have travelled through multiple interfaces and nodes, in addition to the given interface for which the state is being attributed. This also implies that the state of the network encompasses the states of all agents in the environment. 
    %can be noisy and provide incomplete information because in this case the whole state of the network encompasses the states of all agents in the environment. 
    %Moreover, the total reward will also depend on the joint actions of all the agents. The agents neither know the observations other agents have perceived nor can compute the global reward by themselves. 
    %--------------------------
    %However, complete observability is a necessary requirement ({\abde This is a strong statement. Is it really a necessity? If yes, please add a citation @Abu ?} ) for MDP based learning paradigms such as Q-learning and DQN to converge to the optimum solution. 
    %---------------------------
    %If partial observation of the agents is treated as the state of the environment the DQN will have difficulty converging and the agents may eventually learn sub-optimal solutions. 
    %---------------------
    %{\abde \textbf{WHAT WE CAN ADD HERE IS:} 
    %Moreover, agents cannot figure out events beyond their local knowledge including if their available interfaces leading to a given producer are overlapping or no, or if they will compete with other flows using portions of the path towards the producer. All these events may result in similar measured rewards, but require different mitigation (\eg drop packets, choose different interface, etc.) 
    %--------------------------
    %}
    %\todo[inline]{Similar to the previous item, we must use a scenario where if every agent aim at maximizing throughput ``locally'' this does not result in maximizing the overall throughput.}
    

    %\subsection{Multi-Agent RL}
    %\item \textbf{Multi-Agent RL}
    %%We trained the forwarding agents in each router individually independently to achieve a global optimization of network performance. 
    %----------------------
    %The generalization of the MDPs for multi-agent case gives rise to a stochastic game. In the multi-agent case, the state transitions occur as the result of the joint action of all the agents. In our case of stateful forwarding, we need fully cooperative agents with a common goal. The agents can exploit the decentralized structure of the task through experience sharing. This can also help the agents with similar tasks to learn faster and better. For instance, agents can exchange information using communication, skilled agents may serve as teachers for the learner, or the learner may watch and imitate the skilled agents. The information passing among agents will add additional stress to the network and could be perceived as a substitute for the routing algorithm. This will be contrasting to the goal of stateful forwarding that primarily aims to make local forwarding decision with no additional burden on the network traffic.
    %A prominent solution for the convergence of the multi-agent DQNs is that the Q function values of all the agents are shared with a central entity and the globally best Q-value is used by all the agents to update the DNN parameters. However to achieve this in ICN, we need a centralized controller such as the SDN.
    %------------------------
    %\todo[inline]{Context sharing can be done without going as far as implementing an SDN. Do you think that context sharing (agents share states with each others) would help? We must discuss here. SDN is not a distributed solution. We would like to focus our discussion of distributed ML/RL}  
    
%\end{enumerate}


==> Analysis of Independent Learning in Network Agents-A Packet Forwarding Use Case/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%------------------------
%------------------
In this paper, we applied IQL, the autonomous and non-cooperative multi-agent RL approach to perform packet forwarding in NDN. We approximated the Q-function of IQL using DQN. We performed many experiments in different topologies with tuning of several parameters to achieve a better generalization of the DQN. We show that our implemented forwarding scheme, IDQF does not significantly improve the network performance compared to the default forwarding strategy available in NDN. We have also presented several challenges (\eg non-stationarity, partial observability, etc.) of  this approach using examples and experiments to support its effect on the performance of IDQF. A possible direction for our future work is to try fully cooperative multi-agent reinforcement learning approaches to design forwarding strategies. %where agents will share their Q-values among one another through communication to guarantee convergence to their optimal behavior.  

%----------------------
%with respect to the problem of designing a NDN forwarding strategy. %on the convergence properties of DQN. 
%A prominent solution for the convergence of the multi-agent DQNs is that the Q function values of all the agents are shared with a central entity and the globally best Q-value is used by all the agents to update the DQN parameters. However, to achieve this in ICN, we need a centralized controller such as the SDN. Another possible direction for future research is to have the agents exploit the decentralized structure of the task through experience sharing using communication. This can help the agents with to learn faster and better. However, the information passing among agents will add additional stress to the network and could be perceived as a substitute for the routing algorithm. This will be contrasting to the goal of stateful forwarding that primarily aims to make local forwarding decision with no additional burden on the network traffic. 

%The generalization of the MDPs for multi-agent case gives rise to a stochastic game. In the multi-agent case, the state transitions occur as the result of the joint action of all the agents. 
%In our case of stateful forwarding, we need fully cooperative agents with a common goal. The agents can exploit the decentralized structure of the task through experience sharing. This can also help the agents with similar tasks to learn faster and better. For instance, agents can exchange information using communication, skilled agents may serve as teachers for the learner, or the learner may watch and imitate the skilled agents. The information passing among agents will add additional stress to the network and could be perceived as a substitute for the routing algorithm. This will be contrasting to the goal of stateful forwarding that primarily aims to make local forwarding decision with no additional burden on the network traffic.
%A prominent solution for the convergence of the multi-agent DQNs is that the Q function values of all the agents are shared with a central entity and the globally best Q-value is used by all the agents to update the DQN parameters. However to achieve this in ICN, we need a centralized controller such as the SDN.



%\textcolor{red}{Is ML promising for stateful forwarding? What do you recommend?}
%The performance of RL is very poor when the network is relaxed or without any congestion. Even with moderate level of congestion, the BR wins over RL.Talk about Multiple consumers and multiple producers.
%==================================
%In this paper, we explored the viability of several designs of state, reward, and action for proposing a deep reinforcement learning(DRL)-based forwarding strategy which will intelligently forward interest packets to the optimal interface in NDN network. We also tried out some non-machine learning (Non-ML) based stateful strategies that will be operated by network parameter defined objective function. We compared the performance of all our strategies mainly with state-less BestRoute (\emph{BR}) strategy, available as default implementation in \emph{ndnSIM} and some other stateful strategies like ASF and INFORM. From the comparative experiments we conducted, we found that the DRL strategy and other Non-ML strategies do not perform better than \emph{BR} in all network case scenarios.    



==> Analysis of Independent Learning in Network Agents-A Packet Forwarding Use Case/evaluation.tex <==
\section{Performance Evaluation}
\label{subsec:eval}
\subsection{Experiment Setup}
We performed all the simulations using the official NDN project simulator \emph{ndnSIM-2.7}~\cite{mastorakis2017ndnsim,tr-mastorakis2016ndnsim}. To implement DQN network for training the node agents, we developed a program using Python language~\cite{python}. We leveraged a popular library, Keras~\cite{chollet2015keras} that provides a high-level API to TensorFlow~\cite{abadi2016tensorflow} to build the neural networks of DQN. Since it is challenging to run the DQN algorithm inside the \emph{ndnSIM} simulator, we implemented the Python program as a daemon process. This process will always be active and wait for messages to be sent from the nodes inside the simulator. The message formats were defined using a standard platform neutral language called Protocol buffers~\cite{Varda2008}. To actualize the communication system between the simulator and the python program, we exploited ZeroMQ messaging library~\cite{ZeroMQ2011}. The messages usually consists of state or action of a node with its identifier. When a message from a particular node arrives, the daemon process will use the identifier of the node to train its corresponding DQN agent and send back the predicted action of the agent to the node.  
%---------------------------

To evaluate our forwarding strategy in a multi-agent scenario where each node in the network will act as agent and predict the next hop interface we choose the sprint topology. 
This topology consists of $11$ nodes and $18$ links~\cite{Knight-Topology-Zoo}. We consider one consumer and one producer case. Consumer is connected to node `Boulder' and producer is connected to node `Seattle' with 5 Mbps links. While all the other links have 1 Mbps bandwidth, `Boulder'-`Cheyenne' link has 2 Mbps bandwidth, which is also the network capacity. The delays of each link are labeled in Figure~\ref{fig:topo-Sprint-2} and are in milliseconds unit. Every node in the network can hold maximum 100 packets in the transmission queue. We put RL agents in `Cheyenne', `Stockton', `Kansas City', and `Chicago'. 

We evaluate the performance with interest rates of $100$, $300$, and $500$ packets/sec corresponding to three different levels of congestion in the network. The BR strategy runs a routing protocol at the beginning of the simulation and identifies the shortest delay path between a producer and consumer. Therefore, with no congestion 

%--------------------------
\subsection{Handling the re-transmitted packets}
%In our ndnSIM simulation experiments, 
We set the \textit{maximum re-transmission timeout} of consumers to be $1~S$. That means, the consumer will wait maximum $1s$ before re-transmitting an interest packet for which it did not receive any data packet. In this setting, every time an interest packet is re-transmitted, the expiry time of the corresponding PIT entry in consumer gets extended. Since the lifetime of a PIT entry is $2s$, all the PIT entries of the unsatisfied interests in consumer remain alive until satisfied by data packets. However, the concept of re-transmission and activeness of PIT entry is different in intermediate NDN routers. In a NDN router, an interest packet is considered re-transmitted when there exists an unexpired out-record in the PIT entry of that interest. That means, that interest has been forwarded earlier through some interface, but has not been satisfied yet. If the router forwards that interest again through the same interface or another interface, then the lifetime of PIT entry gets extended. But the PIT entry of that interest may expire and get deleted if no interest with the same name and selector is received by the router or the PIT entry is satisfied within its lifetime. Therefore, even if an interest is a re-transmitted packet from the consumers point of view, it may be considered as new interest packet in the router when no PIT entry exists for the interest. 
There are two ways we can handle re-transmitted packets: 
% \begin{enumerate}
% \item \textbf{BR-way of re-transmission:} Consider the interest as a re-transmitted packet and forward it in the same way as BestRoute (BR) does. To forward a re-transmitted interest, BR strategy first tries to find an unused interface. If it can not not find any unused interface, then it uses an interface that has been used earliest.
% \item \textbf{Non-BR-way of re-transmission:} Consider the interest as new packet and forward it through any of the interfaces chosen by the agent.
% \end{enumerate}
(i) {BR-way:} We forward the re-transmitted packet in the same way as the BestRoute (BR) algorithm does. To forward a re-transmitted interest, BR strategy first tries to find an unused interface. If it can not not find any unused interface, then it uses an interface that has been used immediately before.
(ii) {Reward as a function of Re-transmission} We consider the re-transmitted packet as new packet and forward it through an interfaces recommended by the agent.

To evaluate which method of re-transmission is better we conducted an experiment where the average delay of the last $5$ packets and interest satisfaction ratio of each interface were considered as the state vector. The reward was chosen to minimize the average of delays of the data packets received through the last chosen interface between last decision epoch and current decision epoch ($\alpha = 0$). We trained the agents for $50$ episodes with $\delta t = 20$, batch size = 16, and learning rate = 1. In order to simplify the learning task we restricted the number of available next hop interface in FIB (Forwarding Information Base) for each node to $2$. 
\subsubsection{BR-way of re-transmission}
The results with BR-way of re-transmission are summarized in Table~\ref{tab:BR-D-st} for three different interest rates (100, 300, and 500, packets/sec).
%The results with both the ways of re-transmission are summarized in Table~\ref{tab:BR-D-st} and 
%-------------------------
%--------------------------
% \subsubsection{BR-way of re-transmission}
% \label{BR-D-st}
% We performed experiments %on topology of Figure~\ref{fig:topo-Sprint-2} 
% with three different interest rates (100, 300, and 500, packets/sec) using the following experiment setup. 
% We used average delay of the last 5 packets and interest satisfaction ratio per interface as state feature. We define the reward to optimize as average of delays of the data packets received through the last chosen interface between last decision epoch and current decision epoch.  Trained the agents using epsilon-greedy method for $50$ episodes with $\delta t = 20$, batch size = 16, and learning rate = 1. Number of available next hop interface in FIB (Forwarding Information Base) per node were restricted to 2 during training. The results are summarized in Table~\ref{tab:BR-D-st}.
%---------summary-----------
\begin{table}[h!]
  \begin{center}
    \begin{tabular}{|l|l|l|l|l|} % 
    \hline
    \textbf{Interest Rate} & \multicolumn{2}{c|}{\textbf{Total}} & \multicolumn{2}{c|}{\textbf{Avg App}} \\
    \textbf{(pkts/s)} & \multicolumn{2}{c|}{\textbf{Throughput (Mbps)}} & \multicolumn{2}{c|}{\textbf{Delay (ms)}}\\
      \hline
      & BR & RL & BR & RL\\
      \hline
      300 & 1.65 & 1.65 & 1140.68 & 1135.40\\
      \hline
      500 & 1.29 & 1.34 & 2606.40 & 2211.68\\
      \hline
    %   1000 & 1.30 & 1.33 & 4853.65 & 4309.31\\
    %   \hline
    \end{tabular}
    \caption{BR-D-st: Summary results}
    \label{tab:BR-D-st}
  \end{center}
\end{table}
%--------------------------
We found that the total throughput and average delay of both BR and RL strategies remained same. All the four node agents use the minimum delay next hop interface for transmitting the new packets. 

With 300 interest rate the maximum number of re-transmissions per packet from the consumer was one. So BR strategy used only the second ranked next hop interface to forward those packets. Since RL strategy in this experiment utilizes the same mechanism to forward re-transmitted packets, the total throughput and average delay for BR and RL are almost same.  

For $500$ packets/sec, the congestion increases and we observe that the total throughput of RL strategy is $12.4\%$ higher compared to BR strategy. Similarly the average delay of RL strategy is $15.14\%$ lower than that of BR strategy. This is because the BR strategy used some alternate next hop interfaces to forward re-transmitted packets, which causes the data packets to either drop or travel through a longer delay path. For example, Chicago sent some interest packets to Stockton and Kansas City. On the contrary, RL strategy was forced to use only two next hop interfaces. Thus, RL strategy got a small advantage in gaining improved throughput and delay. 

% %-----------------------------
% \subsubsection{300 packets per second ($\approx 2.45~Mbps$)}

% We present the results of this experiment in Figures \vrefrange {fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-performance}{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-nodestat}.
% From Figure~\ref{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-performance}, we find that the total throughput and average delay of both BR and RL strategies are same. Figure~\ref{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-nodestat} shows us that all the four node agents use the minimum delay next hop interface for transmitting the new packets. 
% With 300 interest rate the maximum number of re-transmissions per packet from the consumer is one. So BR strategy uses only the second ranked next hop interface to forward those packets. Since RL strategy in this experiment utilizes the same mechanism to forward re-transmitted packets, the total throughput and average delay for BR and RL are almost same.   

% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-app-delay.pdf}
% \caption{Network Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-app-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--throughput}
% \end{subfigure}
% \caption{BR-D-st:Network Performance 300 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-performance}
% \end{figure}

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--Node4}
% \end{subfigure}
% \caption{BR-D-st:Node statistics for 300 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-nodestat}
% \end{figure}

% %----------------------
% \subsubsection{500 packets per second ($\approx 4~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-performance}{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-nodestat}. In this experiment, we observe that the total throughput of RL strategy is 12.4\% higher compared to BR strategy. Similarly the average delay of RL strategy is 15.14\% lower than that of BR strategy. This is because the BR strategy used some alternate next hop interfaces to forward re-transmitted packets, which causes the data packets to either drop or travel through a longer delay path. For example, Chicago sent some interest packets to Stockton and Kansas City. On the contrary, RL strategy was forced to use only two next hop interfaces. Thus, RL strategy gets slight advantage in gaining better throughput and delay. 

% %-----------------
% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-app-delay.pdf}
% \caption{Network Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-app-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--throughput}
% \end{subfigure}
% \caption{BR-D-st:Network Performance 500 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-performance}
% \end{figure}

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--Node4}
% \end{subfigure}
% \caption{BR-D-st:Node statistics for 500 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-nodestat}
% \end{figure}
% %----------------------------
% %====================
% \subsubsection{1000 packets per second ($\approx 8~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-performance}{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-nodestat}. We observe that with 1000 interest rate RL strategy 
% achieves 14.62\% higher total throughput and 13.86\% lower average delay compared to BR strategy. The is because unlike BR strategy, the RL strategy forwards some new packets through alternative next hop interface instead of using only the minimum delay next hop interface. As a result, in RL strategy packet drops are slightly less than that of BR strategy.    

% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-app-delay.pdf}
% \caption{Network Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-app-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-throughput.pdf}
% \caption{Throughput}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--throughput}
% \end{subfigure}
% \caption{BR-D-st:Network Performance 1000 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-performance}
% \end{figure}

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--Node4}
% \end{subfigure}
% \caption{BR-D-st:Node statistics for 1000 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-nodestat}
% \end{figure}

%---------------------------
\emph{Is BR-way of re-transmission good? :}
One of the problems with BR way of re-transmission is that it may sometimes forward interests through an unused next hop interface which goes along a longer path. Moreover, BR strategy always forwards all new packets to the lowest ranked next hop interface whereas sometimes it is useful to distribute some of the new packets as well as re-transmitted packets to alternate interfaces. If RL strategy follows this mechanism, then there is very little scope for the agent to learn how to distribute the packets in other interfaces. Specially, when interest rate is high, the number of re-transmitted interest packets increase. As a result, the agents will not have enough data for training.    
%=============================
%\subsubsection{Re-transmission as feature}
\subsubsection{Reward as a function of re-transmission}
The motivation to define this feature is to capture the congested situation of a path in the network. Since packets are usually re-transmitted when consumer does not receive data within a specific time, we can use the re-transmission feature to represent the congestion that exists for a next hop interface. Let us represent the re-transmission feature as: 

$\mathbf{R}_t^n = [r_1^n, r_2^n, \cdots r_F^n]$, where $F$ is the number of interfaces available at node $n$ and $r_j^n$ is the re-transmission value for the $j$-th interface at node $n$. When $j$-th interface is chosen in the last decision epoch, re-transmission value can be computed in the following two ways:
    
\begin{enumerate}
    \item Re-transmission ratio:  
    \begin{equation}
    \label{eq:rr}
        r_j^n=
        \begin{cases}
        0, & \text{if}\ R_j<=0 \\
        R_j/R, & \text{otherwise}
        \end{cases}
    \end{equation}
    ,where $R_j$ is the number of packets that were originally transmitted through interface $j$, but re-transmitted through $j$ in the last decision epoch, and $R$ is the total number of re-transmitted packets through $j$ in the last decision epoch. 
     \item Re-transmission difference: 
     \begin{equation}
     \label{eq:rd}
        r_j^n=
        \begin{cases}
        0, & \text{if}\ R-N<0 \\
        R-N, & \text{otherwise}
        \end{cases}
    \end{equation}
    ,where $N$ is the number of new packets transmitted through $j$ in the last decision epoch.
\end{enumerate}
%---------------------
\begin{figure}[ht]
  \centering
  %\includegraphics[scale=.5]{figures/rt_feature.pdf}
  \includegraphics[width=\columnwidth]{figures/rt_feature.pdf}
  \caption{Re-transmission as feature}
  \label{fig:re-transmission feature}
\end{figure}
%------------------------
We illustrate the above terms in Figure~\ref{fig:re-transmission feature}. Let us assume that at time $t$ we need to get a decision from the node agent. In the last decision epoch at time $t-\delta t$, the predicted interface was \textit{Face1}. Assume that among all the packets transmitted between $t$ and $t-\delta t$ through \textit{Face1}, four packets were re-transmitted packets and one packet was a new packet, i.e. $R = 4$ and $N=1$. If out of four packets, three packets were originally transmitted (new) through \textit{Face1} at time $(t-101\times\delta t)$ and one packet was originally transmitted (new) through \textit{Face2} at time $t-103\delta t$, then $R_1 = 3$, $R_2 = 1$, and $R=R_1+R_2$. Now, according to equation \ref{eq:rr}, $r_1^n = 3/4 = 0.75$ and
according to equation \ref{eq:rd},  $r_1^n = 4-1 = 3$.
%----------------------
%=============================
%\clearpage
%\newpage
%========RW-1-2==============
\subsubsection{Non-BR-way of re-transmission} %\textcolor{red}{BEST RESULTS: Reward-1-2}}
\label{NBR-RW1-2}

For this case, we used re-transmission difference in Equation \ref{eq:rd} as extra feature of the state along with the average delay and interest satisfaction ratio features. We chose the reward as: 
    \small
    \begin{equation}
    \label{eq:rw1}
        RW1 =
        \begin{cases}
         -(AvgD + R_{lf}\times CM)    , & \text{if}\ R-N > R_{thrs} \: \text{and} \: AvgD \ne 0 \\
         -(R_{lf}\times CM)    , & \text{if}\ R-N > R_{thrs} \: \text{and} \: AvgD = 0 \\
         -(AvgD), & \text{if}\ R-N \leq R_{thrs} \: \text{and} \: AvgD \ne 0 \\
        -10000, & \text{if}\ R-N \leq R_{thrs} \: \text{and} \: AvgD = 0 
        \end{cases}
    \end{equation}
    \normalsize
to minimize the overall delay in the network.
 where $lf$ is the chosen interface in the last decision epoch, $R_{lf}$ is the number of packets in $R$ which were transmitted through $lf$ last time, $AvgD$ is average delay of the data packets received through interface $lf$ between last decision epoch and current decision epoch, $CM$ is a constant multiplier to make the reward smaller to account for the re-transmitted packets due to packet drops, $R=$ number of
    re-transmitted packets and $N=$ number of new packets in the last decision epoch, $R_{thrs}$ is a threshold. We chose $R_{thrs}=0$ for 300 interest rate and $R_{thrs}=1$ for 500 interest rate, and $R_{thrs}=2$ for 1000 interest rate. In our experiment, we chose different values of $CM \in \{ 1000, 4000, 8000, 20000\}$ and present the results of $CM=4000$. Number of available next hop interface per node were restricted to 2 during training. Trained for 50 episodes with $\delta t = 10$, batch size = 16, and learning rate = 1. We summarize the results in Table~\ref{tab:RD-st-p4s}.

% We performed experiments on topology of Figure~\ref{fig:topo-Sprint-2} with three different interest rates (300, 500, and 1000 packets/sec) using the following experiment setup.  

% \begin{enumerate}
%     \item \textcolor{blue}{Used re-transmission difference in Equation \ref{eq:rd} as extra feature of the state along with the average delay and interest satisfaction ratio features.}
    
%     \item Goal is to minimize the overall delay in the network.
    
%     \item 
%     The reward function for interface $lf$ is the following,
%     \small
%     \begin{equation}
%     \label{eq:rw1}
%         RW1 =
%         \begin{cases}
%          -(AvgD + R_{lf}\times CM)    , & \text{if}\ R-N > R_{thrs} \: \text{and} \: AvgD \ne 0 \\
%          -(R_{lf}\times CM)    , & \text{if}\ R-N > R_{thrs} \: \text{and} \: AvgD = 0 \\
%          -(AvgD), & \text{if}\ R-N \leq R_{thrs} \: \text{and} \: AvgD \ne 0 \\
%         -10000, & \text{if}\ R-N \leq R_{thrs} \: \text{and} \: AvgD = 0 
%         \end{cases}
%     \end{equation}
%     \normalsize
%      where $lf$ is the chosen interface in the last decision epoch, $R_{lf}$ is the number of packets in $R$ which were transmitted through $lf$ last time, $AvgD$ is average delay of the data packets received through interface $lf$ between last decision epoch and current decision epoch, $CM$ is a constant multiplier to make the reward smaller to account for the re-transmitted packets due to packet drops, $R=$ number of
%     re-transmitted packets and $N=$ number of new packets in the last decision epoch, $R_{thrs}$ is a threshold. We chose $R_{thrs}=0$ for 300 interest rate and $R_{thrs}=1$ for 500 interest rate, and $R_{thrs}=2$ for 1000 interest rate. In our experiment, we chose different values of $CM \in \{ 1000, 4000, 8000, 20000\}$ and present the results of $CM=4000$. %in Figures \vrefrange {fig:Time2TDQN-SW32-NoFlowRFace-10-e50r300l60-load20sr300sd180rt=0-tlr=500_perform}{fig:Time2TDQN-SW32-NoFlowRFace-10-e50r500l60-load30sr500sd180rt=1-tlr=500_nodestat}. 
    
%     \item Used Non-BR-way of re-transmission to handle re-transmitted packets. 
    
%     \item Number of available next hop interface per node were restricted to 2 during training.
    
%     \item Trained the agents using epsilon-greedy method for multiple episodes.
    
%     \item Trained for 50 episodes with $\delta t = 10$, batch size = 16, and learning rate = 1. 
    
%     \item  We summarize the results in Table~\ref{tab:RD-st-p4s}.
% \end{enumerate}

%-------------------------
\begin{table}[h!]
  \begin{center}
    \begin{tabular}{|l|l|l|l|l|} % 
    \hline
    \textbf{Interest Rate} & \multicolumn{2}{c|}{\textbf{Total}} & \multicolumn{2}{c|}{\textbf{Avg App}} \\
    \textbf{(pkts/s)} & \multicolumn{2}{c|}{\textbf{Throughput (Mbps)}} & \multicolumn{2}{c|}{\textbf{Delay (ms)}}\\
      \hline
      & BR & RL & BR & RL\\
      \hline
      300 & 1.69 & 1.44 & 1148.42 & 1340.29 \\
      \hline
      500 & 1.31 & 1.75 & 2691.18 & 2121.94\\
      \hline
    %   1000 & 1.31 & 1.30 & 5370.49 & 5963.16 \\
    %   \hline
    \end{tabular}
    \caption{RD-st-p4s: Summary results of RW1}
    \label{tab:RD-st-p4s}
  \end{center}
\end{table}

%--------300------------------
For a data rate of $300$ packets/sec, we find that after 20 seconds of simulation, node agent Cheyenne forwards interest packets 60\%-80\% times through Stockton, the minimum delay next hop and 20\%-40\% times through the KansasCity next hop. The more utilization of the minimum delay next hop and less utilization of the alternate next hop interface causes the RL strategy to achieve total throughput of 1.44 Mbps, which is 6.67\% better than what we achieved when we used the Equation \ref{eq:rr} to compute the re-transmission feature. We conjecture that Equation \ref{eq:rd} better represents the congested state of the network and facilitates frequent switching of the links. Because in Equation \ref{eq:rd}, we are assigning a higher value, $R-N$ to the last chosen interface. That means, we are forwarding more re-transmitted packets and most probably that interface will become congested. On the other hand, in Equation \ref{eq:rr} we assign $R_{lf}$ value which represents a 1 second older congested state of the last chosen interface. 

For a data rate of $300$ packets/sec, we observe that node agent Cheyenne keep switching links from the beginning of the simulation. The almost even utilization of the both Stockton and KansasCity next hop interfaces allowed the RL strategy to achieve total throughput of 1.75 Mbps, which is 33.59\% higher than BR strategy and 8\% better than what we achieved when we used the Equation \ref{eq:rr} to compute the re-transmission feature. We speculate that because of the higher interest rate the number of re-transmissions are higher in this case. As a result, in Equation \ref{eq:rd} the assigned $R-N$ values are higher most of the time. This helps the agent to alternate links frequently considering the congested state of the next hop interfaces. 

% \subsubsection{300 packets per second ($\approx 2.45~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-performance}{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-debug-rtt-pnlt-summ}.

% From Figure~\ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node3}
% we find that after 20 seconds of simulation, node agent Cheyenne forwards interest packets 60\%-80\% times through Stockton, the minimum delay next hop and 20\%-40\% times through the KansasCity next hop. The more utilization of the minimum delay next hop and less utilization of the alternate next hop interface causes the RL strategy to achieve total throughput of 1.44 Mbps, which is 6.67\% better than what we achieved when we used the Equation \ref{eq:rr} to compute the re-transmission feature. We conjecture that Equation \ref{eq:rd} better represents the congested state of the network and facilitates frequent switching of the links. Because in Equation \ref{eq:rd}, we are assigning a higher value, $R-N$ to the last chosen interface. That means, we are forwarding more re-transmitted packets and most probably that interface will become congested. On the other hand, in Equation \ref{eq:rr} we assign $R_{lf}$ value which represents a 1 second older congested state of the last chosen interface. 

%-------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-net-delay.pdf}
% \caption{Network Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-net-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-net-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-net-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--throughput}
% \end{subfigure}
% \caption{RD-st-p4s:Network Performance 300 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-performance}
% \end{figure}
% %-------------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node4}
% \end{subfigure}
% \caption{RD-st-p4s:Node statistics for 300 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-nodestat}
% \end{figure}
%-----------------debugging---------
% \begin{figure}[h!]
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Cheyenne-rtt-pnlt-summ.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-Node3-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-KansasCity-rtt-pnlt-summ.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-Node6-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Stockton-rtt-pnlt-summ.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-Node9-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Chicago-rtt-pnlt-summ.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-Node4-rtt-pnlt-summ}
% \end{subfigure}
% \caption{RD-st-p4s:Time vs Condition Satisfied for 300 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-debug-rtt-pnlt-summ}
% \end{figure}

% %--------------500--------------
% \subsubsection{500 packets per second ($\approx 4~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-performance}{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-debug-rtt-pnlt-summ}.

% From Figure~\ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node3}
% we observe that node agent Cheyenne keep switching links from the beginning of the simulation. The almost even utilization of the both Stockton and KansasCity next hop interfaces allowed the RL strategy to achieve total throughput of 1.75 Mbps, which is 33.59\% higher than BR strategy and 8\% better than what we achieved when we used the Equation \ref{eq:rr} to compute the re-transmission feature. We speculate that because of the higher interest rate the number of re-transmissions are higher in this case. As a result, in Equation \ref{eq:rd} the assigned $R-N$ values are higher most of the time. This helps the agent to alternate links frequently considering the congested state of the next hop interfaces. 

% %-----------------
% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-net-delay.pdf}
% \caption{Network Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-net-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-net-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-net-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--throughput}
% \end{subfigure}
% \caption{RD-st-p4s:Network Performance 500 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-performance}
% \end{figure}
% %--------------------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node4}
% \end{subfigure}
% \caption{RD-st-p4s:Node statistics for 500 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-nodestat}
% \end{figure}
%-----------------debugging---------
% \begin{figure}[h!]
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Cheyenne-rtt-pnlt-summ.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-Node3-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-KansasCity-rtt-pnlt-summ.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-Node6-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Stockton-rtt-pnlt-summ.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-Node9-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Chicago-rtt-pnlt-summ.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-Node4-rtt-pnlt-summ}
% \end{subfigure}
% \caption{RD-st-p4s:Time vs Condition Satisfied for 500 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-debug-rtt-pnlt-summ}
% \end{figure}

%----------1000-----------------
% \subsubsection{1000 packets per second ($\approx 8~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-performance}{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-debug-rtt-pnlt-summ}.

% From Figure~\ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node3}, \ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node4}, and \ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node9}, we find that from the beginning of the simulation, node agents Cheyenne, Stockton, and Chicago forward interest packets through both of their next hop interfaces. Because of the higher interest rate, experience replay memory fills up with transition samples from both hops. Since lots of re-transmissions occur in all three nodes and the reward is defined as a function of the number of re-transmissions, the DQN network of the nodes update their parameters frequently. Moreover, in Equation \ref{eq:rd} the assigned $R-N$ values are higher most of the time, which also helps the agent to capture the congested state of the next hops and alternate links. Due to the higher data rate lots of packets drop at Stockton and Chicago in addition to Seattle. Therefore, the throughput oscillates between 0.9 Mbps and 1.7 Mbps.
% %----------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-net-delay.pdf}
% \caption{Network Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-net-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-net-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-net-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-throughput.pdf}
% \caption{Throughput}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--throughput}
% \end{subfigure}
% \caption{RD-st-p4s:Network Performance 1000 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-performance}
% \end{figure}
% %------------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node4}
% \end{subfigure}
% \caption{RD-st-p4s:Node statistics for 1000 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-nodestat}
% \end{figure}
%--------------------------
\subsubsection{\textcolor{blue}{Training duration (short vs long)}}
In this experiment, we compared the performance of two RL models trained with different lengths of simulation. We trained each model for $50$ episodes with $60$ and $500$ seconds per episode. %In Figure~\ref{fig:RD-st-p4s-500-Short-Long-performance}, \textit{RL-Ep50-L60} refers to the model which has been trained 60 seconds per episode and \textit{RL-Ep50-L500} refers to the model which has been trained $500$ seconds per episode. 
%--------500----------
If we compute the total throughput and average delay for the steady state of the network, i.e. ignoring the data of first 20 seconds of simulation, %we find that \textit{RL-Ep50-L60} 
we found that the model trained for $60$ seconds/episodes achieves $7.2\%$ higher throughput and $6.4\%$ less average application delay compared to the model trained for $500$ seconds/episodes. %\textit{RL-Ep50-L500} model.  
%--------300--------
%If we compute the total throughput and average delay for the steady state of the network, i.e. ignoring the data of first 20 seconds of simulation, we find that \textit{RL-Ep50-L60} model achieves 3.4\% higher throughput and 10.49\% less average application delay compared to the \textit{RL-Ep50-L500} model.  


% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:Multi-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:Multi-Rt500-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 500 interest rate (Short vs Long duration)}
% \label{fig:RD-st-p4s-500-Short-Long-performance}
% \end{figure}

% %-----------300----------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:Multi-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:Multi-Rt300-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 300 interest rate (Short vs Long duration)}
% \label{fig:RD-st-p4s-300-Short-Long-performance}
% \end{figure}

%----------------------
\subsubsection{\textcolor{blue}{One vs Multi Episode Training:}}

In this experiment, we compare performance of two RL models, one trained with $50$ episodes of $60$ seconds  duration and another with one episode of $6000$ seconds duration. Comparing the steady state (discarding first 20 seconds of simulation) data, We observed that the model with $50$ episodes achieves $33.6\%$ higher throughput and 25.4\% less application delay compared to the model with one long episode.
%In Figure~\ref{fig:RD-st-p4s-One-Multi-performance}, \textit{RL-Ep50-L60} refers to the model which has been trained for 50 episodes where duration of each episode was 60 seconds and \textit{RL-Ep1-L6000} refers to the model which has been trained for one episode where duration of the single episode was 6000 seconds. Computing the total throughput and average delay for the steady state of the network (discarding first 20 seconds of simulation data), we find that \textit{RL-Ep50-L60} model achieves 33.6\% higher throughput and 25.4\% less application delay compared to the \textit{RL-Ep1-L6000} model.   

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-vs-One-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:Multi-vs-One-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-vs-One-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:Multi-vs-One-Rt500-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 500 interest rate (One vs Multi Episode)}
% \label{fig:RD-st-p4s-One-Multi-performance}
% \end{figure}

% %---------------300-----------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-vs-One-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:Multi-vs-One-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-vs-One-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:Multi-vs-One-Rt300-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 300 interest rate (One vs Multi Episode)}
% \label{fig:RD-st-p4s-300-One-Multi-performance}
% \end{figure}

%---------------
\subsubsection{\textcolor{blue}{Low vs High learning rate:}}

In this experiment, we compare performance of two RL strategy models tested with different learning rates \textcolor{red}{is it the Q-value update learning rate or the DNN weight update learning rate}. We chose two learning rates of $100$ and $500$. These values were chosen by a trial-and-error approach. %In Figure~\ref{fig:RD-st-p4s-300-Low-High-performance}, \textit{Ep50-L60-LR100} refers to the model which has been tested with learning rate $100$ and \textit{Ep50-L60-LR500} refers to the model which has been tested with learning rate 500. 
Both models were trained for $50$ episodes with $60$ seconds of simulation per episode. Comparing the steady state performance we observed that the model with a learning rate of $500$ achieves $38.53\%$ higher throughput and $57.47\%$ less application delay compared to the model with a learning rate of $100$.
%Computing the total throughput and average delay for the steady state of the network (discarding first 20 seconds of simulation data), we find that \textit{Ep50-L60-LR500} model achieves 38.53\% higher throughput and 57.47\% less application delay compared to the \textit{Ep50-L60-LR100} model. 

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/LearningRate-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:LearningRate-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/LearningRate-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:LearningRate-Rt300-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 300 interest rate (Low vs High Learning rate)}
% \label{fig:RD-st-p4s-300-Low-High-performance}
% \end{figure}

% %----------500--------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/LearningRate-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:LearningRate-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/LearningRate-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:LearningRate-Rt500-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 500 interest rate (Low vs High Learning rate)}
% \label{fig:RD-st-p4s-500-Low-High-performance}
% \end{figure}
% %------------------
%\subsubsection{\textcolor{blue}{Heterogeneity between training and deployment:}}
% In this experiment, we compare performance of two RL strategy models tested with different learning rates. In Figure~\ref{fig:RD-st-p4s-300-Same-Different-performance} and Figure~\ref{fig:RD-st-p4s-500-Same-Different-performance}, \textit{Ep50-L60-CG6-LR500} refers to the model which has been trained with learning rate 1 and tested with learning rate 500 and \textit{Ep50-L60-CG5-LR500} refers to the model which has been trained and tested with learning rate 500. Both models were trained for 50 episodes with 60 seconds of simulation per episode. Computing the total throughput and average delay for the steady state of the network (discarding first 20 seconds of simulation data), we find that \textit{Ep50-L60-CG6-LR500} model achieves 13.73\% and 30.51\% higher throughput for 500 and 300 interest rate respectively compared to the \textit{Ep50-L60-CG5-LR500} model. Also, \textit{Ep50-L60-CG6-LR500} model obtains 12.66\% and 28.75\% less application delay for 500 and 300 interest rate respectively compared to the \textit{Ep50-L60-CG5-LR500} model. 

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct27/LR2-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:LearningRate2-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct27/LR2-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:LearningRate2-Rt300-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 300 interest rate (Same vs Different Learning rate)}
% \label{fig:RD-st-p4s-300-Same-Different-performance}
% \end{figure}

% %----------500--------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct27/LR2-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:LearningRate2-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct27/LR2-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:LearningRate-Rt500-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 500 interest rate (Same vs Different Learning rate)}
% \label{fig:RD-st-p4s-500-Same-Different-performance}
% \end{figure}

%==========================



%--------------------------
\begin{figure}[htbp]
  \centering
  %\includegraphics[width=\textwidth,height=8cm]{figures/sprint2-wcp.pdf}
  \includegraphics[scale=0.6]{figures/sprint-2-ann.pdf}
  %\includegraphics[scale=.5]{figures/SPRINT_marked_v1.pdf}
  \caption{Sprint topology} 
  \label{fig:topo-Sprint-2}
\end{figure}

\subsection{\textcolor{blue}{Comparison with BR}}
We trained RL strategy model for 500 interest rate and tested that model with simulations of different interest rates. The model was trained for 50 episodes with 60 seconds of simulation per episode.  In Figure~\ref{fig:RD-st-p4s-500-model-test} we show the percentage improvement of throughput and average application delay for different interest rates compared to \emph{bestroute} strategy. We found that when the data rate is almost double (3.3$\sim$4 Mbps) the capacity (2 Mbps) of the network, only then we get 16\%-30\% increase in throughput and 9\%-19\% decrease in average application delay compared to bestroute. When data rate is lower or close to 2 Mbps, in those cases performance degrades 46\%-117\%. 

\begin{figure}[h!]
\includegraphics[width=\linewidth]{figures/RateComp.pdf}
\caption{RD-st-p4s: Network Performance of different interest rates with One trained model}
\label{fig:RD-st-p4s-500-model-test}
\end{figure}
%------------------

==> Analysis of Independent Learning in Network Agents-A Packet Forwarding Use Case/introduction.tex <==
\section{Introduction}
\label{sec:intro}
% A paragraph for each.
% \begin{itemize}
%     \item Distributed RL
%     \item Can we use it for networking/forwarding? 
%     \item Why did we use NDN? We consider the ICN forwarding process, which is a distributed decision process where each node selects the best interface(s)--\ie best next hop(s)--to forward each Interest packet. This process can be modeled as a Markov Decision Process (MDP), which can benefit from reinforcement learning features to hypothetically improve forwarding efficiency.
%     \item Contributions.
% \end{itemize}
%=============OLD TEXT========================
%Reinforcement learning (RL)~\cite{sutton1998introduction} is a machine learning approach that does not require external supervision to learn, just does exploration and interaction with local environment to acquire knowledge. Multi-agent RL has often been proposed and suggested as the ultimate solution to solving complex problems that require cooperative control in distributed systems. However, research that quantitatively assess the benefits of such multi-agent RL in distributed systems are often limited to theoretical models~\cite{jin2018real}, or control environments and systems~\cite{kazmi2019multi}. 
%==================================
Reinforcement learning (RL)~\cite{sutton1998introduction} helps explore and interact with local environment to acquire knowledge to solve real-world problems, especially complex multi-agent systems such as traffic signal control~\cite{wei2019presslight}, controlling drones~\cite{hung2016q}, robot soccer~\cite{schwab2018zero}, machines in factories~\cite{kazmi2019multi}, and automated trading~\cite{jin2018real}. RL-based solutions often deploy (i) a single centralized agent~\cite{stampa2017deep}, or (ii) multiple cooperative agents~\cite{gupta2017cooperative} to acquire the knowledge of such distributed systems. While these solutions may not scale for large distributed systems due to the amount of data exchange (\ie overhead), and additional command and control delays, we investigate in this paper the efficacy of non-cooperative/autonomous agents approach, Independent Q-Learning (IQL)~\cite{tan1993multi, wei2019presslight} and quantitatively and qualitatively assess its performance %of one of the
using packet forwarding in an ISP-scale network as a use-case.   


%is a machine learning paradigm that does not require external supervision to learn, just enables an agent to explore and interact with local environment to acquire knowledge. Many real-world problems such as traffic signal control~\cite{wei2019presslight}, controlling drones~\cite{hung2016q}, robot soccer~\cite{schwab2018zero}, machines in factories~\cite{kazmi2019multi}, automated trading~\cite{jin2018real} can be naturally considered as multi-agent systems. Modelling and quantitative evaluation of all these applications are often limited to using either a centralized agent or cooperative agents. However, in distributed systems for many problems centralized agent is not suitable and cooperative agents sometimes contrast with the goal of the application. 
%In this paper, we adopt the non-cooperative/autonomous agents approach, Independent Q-Learning (IQL)~\cite{tan1993multi, wei2019presslight} and quantitatively and qualitatively assess its performance %of one of the
%using packet forwarding in Named Data Networking (NDN) as an use-case application.   

%----------------------------------
%--------------------------
%where routers leverage stateful nature of the forwarding plane and multiple interfaces to improve data delivery performance.
%-----------------------
%==========OLD TEXT=================
%In this paper, we discuss the benefits of autonomous multi-agent RL approaches for distributed systems such as packet forwarding in distributed networks. As communication networks continue to expand and become more complex 
% day by day
%,using a central entity or SDN to control packet forwarding of all routers turns out to be an infeasible solution. A more scalable and efficient solution is to adopt decentralized multi-agent learning approaches where each router agent in the network will utilize localized information to independently learn making forwarding decisions and try to optimize the network performance. In packet forwarding, agents will be placed at each router (or node). Each agent measures its incoming, outgoing traffic state and learns the best forwarding action using a reward system. In contrast with IP architectures, where stateless routers require external hardware and/or resources to perform RL algorithms, we choose Named Data Networking (NDN) for an easy deployment and assessment. NDN uses a forwarding plane that enables each node to easily deploy a stateful forwarding scheme to select forwarding interfaces independent of the routing algorithm, using networking and application information available at the network layer (a short NDN primer and a motivation behind our NDN choice is provided in section~\ref{sec:motiv}). 
%================================
ISP networks are often large-scale and complex, which renders using (i) a single centralized agent (\eg SDN), or (ii) multiple cooperative agents (\eg message exchange among routers) very costly--large overhead, single/multiple point of failure, and hard to maintain/upgrade. 
%As communication networks continue to expand and become more complex, using a central entity (\eg SDN) to control packet forwarding of all routers turns out to be an infeasible solution. On the other hand, considering each router as separate agents and making them control packet forwarding through cooperation among one another will incur extra communication cost and burden to the networks. 
We assess the potential benefits and efficacy of using independent agents that learn to make forwarding decisions using only localized information (\eg incoming, outgoing traffic state). We choose to implement all our IQL-based models using Named Data Networking (NDN), which provides many ``useful'' features such as an easy to use forwarding plane, and context awareness decisions at the routers, to test our models, configurations, and tuning parameters. We provide a  short NDN primer and a motivation behind our NDN choice in Section~\ref{sec:motiv}. However, we believe that the paper's discussions, outcomes, and conclusions remain valid for IP architecture networks.  

%A more scalable and efficient solution is to treat each router in the network as independent agents and let them learn to make forwarding decisions only utilizing localized information (\eg incoming, outgoing traffic state) and try to optimize the network performance. In contrast with IP architectures, where stateless routers require external hardware and/or resources to perform RL algorithms, we choose NDN architecture for an easy deployment and assessment. NDN uses a forwarding plane that enables each node to easily deploy a stateful forwarding scheme to select forwarding interfaces independent of the routing algorithm, using networking and application information available at the network layer (a short NDN primer and a motivation behind our NDN choice is provided in section~\ref{sec:motiv}). 
%We choose IQL-based method to design a NDN forwarding scheme and evaluate its performance.
%=================================
%We use NDN as a testing platform to implement and test the multi-agent RL forwarding scheme. 
%--------------------------
% While most of the multi-agent RL approaches require information exchange (\eg sharing parameters, states) between agents, 
% %to guarantee their convergence to optimal behavior, %these methods incurs communication costs and synchronization problems. 
% these methods are not suitable for adaptive forwarding in NDN. Because information passing among  router agents will incur communication costs and  synchronization problems. This  will be  contrasting to  the goal of NDN's stateful forwarding that primarily allows routers to make local forwarding decisions using available computed routes with no additional burden on the network.
%-----------------------------------

%In a real-world network with a good number of routers, it is computationally inefficient and unscalable to use a central controller such as SDN for learning forwarding decisions of all routers.
% \textcolor{blue}{As communication networks continue to expand and become more complex day by day, using a central entity similar to SDN to control packet forwarding of all routers turns out to be an infeasible solution. A more scalable and efficient solution is to adopt decentralized multi-agent learning approaches where each router agent in the network will utilize localized information to independently learn making forwarding decisions and try to optimize the network performance.}
% To deal with these issues, a preferred approach is decentralized learning, where each agent is trained independently from others and takes autonomous decisions. %for itself. 
%The independent agents category or IQL is an approach where each agent exclusively uses its own history of partial observations and local rewards to learn, and considers other agents as part of the environment~\cite{wei2019presslight}. 
%----------------------------
 %While most of the decentralized multi-agent RL approaches~\cite{gupta2017cooperative} require information exchange (\eg sharing parameters, states, actions, rewards) between agents, these methods are not suitable for adaptive forwarding in NDN. Because information passing among  router agents will incur communication costs and synchronization problems (\eg coherently choosing individual actions of all agents such that the resulting joint action is optimal). 
%-----------------------------------
%Moreover, router coordination  will be contrasting to the goal of NDN's stateful forwarding mechanism that primarily allows routers to make local forwarding decisions using available computed routes with no additional burden (\eg recomputing routes) on the network.
%---------------------------------
%\textcolor{red} {WHY IQL WAS CHOSEN? IS THIS THE ONLY METHOD?}
%\abde{This is still not enough to justify teh use of IQL. Maybe we chould change the title and the story of the paper and say that we just studied IQL and thi spaper will only evluate if IQL is good or no for distributed forwarding. What's your opinion?}
%-------------------------------------
%===========OLD TEXT=================
% Therefore, we choose the autonomous %non-collaborative 
% multi-agent RL approach, Independent Q-Learning (IQL)~\cite{tan1993multi, wei2019presslight} and quantitatively and qualitatively assess its performance using NDN forwarding scheme as a distributed multi-agent autonomous decision making use-case. 

% In the IQL method, agents are implemented at each network router. The agents construct state by collecting local information regarding incoming and outgoing packets and communication flows, take action of choosing appropriate interface to forward packets, and receive local rewards to learn to make optimal forwarding decisions. However, in a real-world network involving a number of routers and communication flows,  the size and complexity of state-action pairs can be very large, which poses a significant challenge for IQL 
% %Q-learning based IQL method 
% to learn the optimal decision policy. To resolve this challenge in the IQL method, non-linear data driven model such as a neural networks are employed due to their ability to achieve generalization in the presence of multiple complex interactions.
%====================================
%{\abde I am not sure what this paragraph is about and how to connect it with our story. If it is an obvious choice within IQL then I suggest that we talk about it in section III, but if it is yet another choice we've made (and we didn't try other options) then this needs more explanation and discussion} 
% In the IQL method, agents are implemented at each network router. The agents construct state by collecting local information regarding incoming and outgoing packets and communication flows, take action of choosing appropriate interface to forward packets, and receive local rewards to learn to make optimal forwarding decisions. However, in a real-world network involving a number of routers and communication flows, the size and complexity of state-action pairs can be very large, which poses a significant challenge for Q-learning based approach IQL to learn the optimal decision policy. To resolve this challenge in the IQL method, non-linear data driven model such as a neural networks are employed due to their ability to achieve generalization in the presence of multiple complex interactions.
%--------------------------------
%--------------------------------
%A limitation of the IQL is that each agent runs a separate Q-learning algorithm. As a result, the size and complexity of the Q-table may increase enormously for state-action pairs encountered in our problem of packet forwarding, due to the network dynamics. This poses a significant challenge to learn the optimal policy. A deep neural network, due to its ability to achieve generalization in the presence of multiple complex interactions, is deployed to resolve this challenge and learn the optimal policy by approximating the dynamic action-value function. 
%This approach of IQL combined with the deep neural network is referred to as Deep-Q-Network~(DQN)~\cite{mnih2013playing}.
%---------------------
%------------------------------

We compare the performance of a neural network equipped IQL-based forwarding strategy, IDQF (Independent  Deep  Q-Network Forwarding) against the most basic (\ie the simplest) forwarding scheme in NDN, namely {\em best\_route} (BR)~\cite{yi2013case}. We show that BR outperforms IDQF in most of the scenarios by simply choosing one path, while IDQF often fails to select the most appropriate path towards the producer.  

This comparison mainly aims at highlighting the challenges of IQL-based approach in such environment. We ran multiple experiments with various parameters, tuning, and setups to outline the challenges that led to unsuccessful decisions made by IDQF. The identified challenges (not a complete list) include: (i) the non-stationarity of the system due to the lack of global synchronization leading to triggered changes as soon as one agent changes its policy; (ii) the generalization of the training setup that is difficult due to network delays and frequent changes in the environment; (iii) the inability to assess the reward of an action immediately due to the variations of network delays; and %the unavailability of instantaneous rewards due to variations of the delays between an action and its reward measurements; and 
%(iv) the partial observability that limits the decisions to phenomenon which can exclude overlapping paths, conflicting flows, etc.
(iv) the partial observability that prevents the routers to see overlapping paths, conflicting flows, etc. and make optimal decisions.
\textcolor{black}{We discuss these challenges in detail and present experiments and/or examples to support the impact of these challenges on the performance of  IDQF in particular, and distributed autonomous multi-agent RL schemes in general.} 


The rest of this paper is organized as follows. Section~\ref{sec:motiv}
includes background and related works for this work. Section~\ref{sec:RL} summarizes the design of the IDQF forwarding mechanism and describe the simulation results. In Section~\ref{sec:challenge}, \textcolor{black}{we discuss the challenges regarding the IDQF forwarding scheme and autonomous multi-agent RL schemes.} Finally, Section~\ref{sec:conclusion} concludes the paper and suggest future work.

%%==============================
% Unlike, IP communication architecture, information-centric networking (ICN) advocates hierarchical name based communication. In ICN, content objects are uniquely identified by name and clients or consumers request them using Interest packets. The network routers forward the Interest packets toward a provider which holds a permanent or transient copy of the content and trigger delivery of the content using Data packets following the reverse path of the Interest packets. The routers in ICN are characterized by stateful and adaptive forwarding plane which keeps per-hop state through pending interest table (PIT) data structure. This allows each router to make its own decision to forward the Interest packets towards a copy of the consumer's requested content. Since Interest packets cannot loop, routers can utilize multiple paths or interfaces to send interests. The stateful nature of the forwarding plane also enables the routers to measure performance of different paths, rapidly detect failures and retry alternative paths. A smart forwarding scheme at these routers should be able to efficiently utilize all the communication paths to forward packets and optimize the performance utility of the network.

% %\subsection{Motivation}

% Most of the existing forwarding strategies rely on some control heuristics or fixed rules to model the network. However, in real-world these simplified models of network can become inaccurate and unrealistic
% since they overlook many important features, such as
% dynamically changing network conditions and application demands. Therefore,
% the existing solutions to forwarding fail to achieve the optimal performance. 

% The contemporary advancements in Machine Learning (ML) techniques have resulted in traceable solutions for many data intensive applications such as object detection, controlling robots etc.. The central dogma is based on the data driven leaning and the goal is to achieve sufficient generalization of the system behavior from discrete set of observations. This is coherent with the goal of stateful forwarding of interest packets, in a way so that the data packets reach the clients with the objective of optimizing the network performance. 

% The supervised ML algorithms are known to be efficient for data-driven learning, but require an exhaustive training data-set consisting of input and ground truths as output. The key elements of supervised ML are \emph{neural networks}, that are trained by minimizing the error between the output of the networks and the actual output inferred by the input-output pair in the training data-set. For Interest packet forwarding in ICN, such a strategy is not appropriate due to dynamic nature of the network and the lack of exhaustive training data to reach generalization. 

% The Reinforcement Learning (RL) is the branch of ML that focuses on direct learning of the control agents from high-dimensional sensory data~\cite{mnih2013playing}. %Unlike supervised ML, RL does not require a ground truths/teacher to be trained.
% The RL algorithms learn from \emph{rewards} associated with different actions, unlike supervised ML where the inputs and outputs are directly associated. From the perspective of forwarding in ICN, the RL appears to be a vigorous contender. The intelligent agents trained by RL algorithm, may be placed in each router to make forwarding decision with an objective to either minimize the network delay or maximize the network throughput. However, the performance of the RL depends on several factors such as the input sensory data from the observation space, dynamics of the environment, the RL model, tuning of parameters, and the learning algorithm. A critical question is: \emph{What is the potential of RL for stateful intelligent forwarding in ICN?}  

% The contributions of this article are:
% \begin{itemize}
%     \item We present an evaluation of RL strategies for stateful forwarding in NDN
%     \item study the impact of parametric changes on the RL agent behaviour and convergence %key challenges or limitations associated with RL 
%     \item summarize the key challenges and identify the opportunities that RL could offer for intelligent forwarding.
%     %\item distributed optimization, 
% \end{itemize}


%%%%%%%%%%%%% OLD TEXT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Today's IP architecture is designed to deliver data to given addresses, while NDN framework focuses on retrieving data of given names. For end-to-end delivery of packets, IP performs two phases of operation. In the first phase, control plane of the routers construct a forwarding table by exchanging routing updates with neighbors and selecting the best path. In the second phase, data plane of the routers forward packets by inspecting the forwarding table. Thus, routing in IP is \emph{stateful} and adaptive to network changes (e.g. link failure, new or alternative routes), whereas IP forwarding is stateless and cannot adapt to anything unless the control plane instructs. This traditional approach of IP puts the responsibility of data delivery solely on the routing system and is referred to as \textit{smart routing, dumb forwarding}.
%------------------------
% In NDN, routing serves the same purpose as in IP i.e. builds forwarding information base (FIB) by finding the reachability information about permanent copies of different content items stored in producers. Instead of advertising prefixes of IP addresses, NDN routing protocols~\cite{wang2012ospfn, hoque2013nlsr} distribute the name prefixes of the content items. However, forwarding plane of NDN adds per-hop state through pending interest table (PIT) data structure. This allows each router to make its own decision to forward  interest packets towards a copy of the consumer's requested content. Since NDN packets cannot loop, routers can utilize multiple paths or interfaces to send interests. The state-ful nature of the forwarding plane also enables NDN routers to measure performance of different paths, rapidly detect failures and retry alternative paths. This unique feature of NDN is known as \textit{adaptive forwarding}~\cite{yi2012adaptive}.
%-----------------------------
%Information-Centric Network (ICN) architectures, including Named Data Networking (NDN), were mainly designed with focus on caching popular content and disseminate data by requesting content name through packets called Interests, independently of their locations. 
%The forwarding plane of NDN adds per-hop state through pending interest table (PIT) data structure. This allows each router to make its own decision to forward  interest packets towards a copy of the consumer's requested content. Since NDN packets cannot loop, routers can utilize multiple paths or interfaces to send interests. The stateful nature of the forwarding plane also enables NDN routers to measure performance of different paths, rapidly detect failures and retry alternative paths. Leveraging the network state gathered at these routers to make efficient forwarding decisions still remains an important research topic.
%----------------------------
%These decisions are made possible via the forwarding plane that keeps state of the Interests received and satisfied by each interface of a given node. Leveraging the networking data gathered at these nodes to make efficient forwarding decisions remains an important research topic.%largely unexplored~\cite{willFindAcitation}.
%--------------------------------
%The contemporary advancements in Machine Learning (ML) has resulted in traceable solutions for many data intensive applications. The central dogma is based on the data driven leaning and the goal is to achieve sufficient generalization of the system behavior from discrete set of observations. This is coherent with the goal of packet forwarding, where the data packets are forwarded from one node to another with the objective to minimize the overall transmission delay and maximize the chances of packet delivery. 

%The supervised ML algorithms are known to be efficient for data-driven learning, but require an exhaustive training data-set consisting of input and ground truths as output. The key elements of supervised ML are \emph{neural networks}, that are trained by minimizing the error between the output of the networks and the actual output inferred by the input-output pair in the training data-set. For packet forwarding in NDN, such a strategy may not be appropriate due to dynamic nature of the network and the lack of exhaustive training data to reach generalization. 

%The Reinforcement Learning (RL) is the branch of ML that focuses on direct learning of the control agents from high-dimensional sensory data~\cite{mnih2013playing}. The RL algorithms learn from \emph{rewards} associated with different actions, unlike supervised ML where the inputs and outputs are directly associated. From the perspective of forwarding in NDN, the RL appears to be a vigorous contender. The intelligent agents may be placed in each router and trained by RL to take forwarding decision with an objective to either minimize the transmission delay or the network throughput. However, the performance of the RL depends on several factors such as the input sensory data from the observation space, the RL model, proper choice of parameters, and the learning algorithm.

%The prime focus of this paper is to analyze state, action, reward design principles of a reinforcement learning based forwarding strategy, quantify its gain against the state-of the-art strategy and  discuss the issues of deployment. We explore different designs of state and reward function of a RL algorithm called DQN (Deep Q-Network) to implement this forwarding strategy that we name.  strategy will dynamically learn complex network characteristics through training and when deployed will choose the most suitable interface for forwarding Interest packets such that the award (\textit{e.g.} total throughput) is maximized. 
%\sol logs, for each interface, the delay, throughput, and success ratio measurements to tune its forwarding decisions. 
%We consider two use-case topologies to qualitatively and quantitatively compare the performance of RL-based forwarding strategy and best-route strategy (BR for short). We also apply the use-cases to drive the discussion on the trade-offs between efficiency and cost (size of the state vectors at the routers).



% evaluate the performance of RL in packet forwarding and identify the optimal settings for RL deployment. The two main questions we attempt to find answer for are: (1) Do the data driven forwarding approaches based on ML perform better than the state of the art algorithms? (2) How does the choice of parameters effect the performance?
%--------------------------------------------
% RL algorithms, on the other hand, must be able to learn from a scalar reward
% signal that is frequently sparse, noisy and delayed. The delay between actions and resulting rewards,
% which can be thousands of timesteps long, seems particularly daunting when compared to the direct
% association between inputs and targets found in supervised learning. Another issue is that most deep
% learning algorithms assume the data samples to be independent, while in reinforcement learning one
% typically encounters sequences of highly correlated states. Furthermore, in RL the data distribution changes as the algorithm learns new behaviours, which can be problematic for deep learning
% methods that assume a fixed underlying distribution.
%--------------------------------------------


==> Analysis of Independent Learning in Network Agents-A Packet Forwarding Use Case/related_work.tex <==
\section{Related work}

==> evaluation.tex <==
\section{Performance Evaluation}
\label{subsec:eval}
\subsection{Experiment Setup}
We performed all the simulations using the official NDN project simulator \emph{ndnSIM-2.7}~\cite{mastorakis2017ndnsim,tr-mastorakis2016ndnsim}. To implement DQN network for training the node agents, we developed a program using Python language~\cite{python}. We leveraged a popular library, Keras~\cite{chollet2015keras} that provides a high-level API to TensorFlow~\cite{abadi2016tensorflow} to build the neural networks of DQN. Since it is challenging to run the DQN algorithm inside the \emph{ndnSIM} simulator, we implemented the Python program as a daemon process. This process will always be active and wait for messages to be sent from the nodes inside the simulator. The message formats were defined using a standard platform neutral language called Protocol buffers~\cite{Varda2008}. To actualize the communication system between the simulator and the python program, we exploited ZeroMQ messaging library~\cite{ZeroMQ2011}. The messages usually consists of state or action of a node with its identifier. When a message from a particular node arrives, the daemon process will use the identifier of the node to train its corresponding DQN agent and send back the predicted action of the agent to the node.  
%---------------------------

To evaluate our forwarding strategy in a multi-agent scenario where each node in the network will act as agent and predict the next hop interface we choose the sprint topology. 
This topology consists of $11$ nodes and $18$ links~\cite{Knight-Topology-Zoo}. We consider one consumer and one producer case. Consumer is connected to node `Boulder' and producer is connected to node `Seattle' with 5 Mbps links. While all the other links have 1 Mbps bandwidth, `Boulder'-`Cheyenne' link has 2 Mbps bandwidth, which is also the network capacity. The delays of each link are labeled in Figure~\ref{fig:topo-Sprint-2} and are in milliseconds unit. Every node in the network can hold maximum 100 packets in the transmission queue. We put RL agents in `Cheyenne', `Stockton', `Kansas City', and `Chicago'. 

We evaluate the performance with interest rates of $100$, $300$, and $500$ packets/sec corresponding to three different levels of congestion in the network. The BR strategy runs a routing protocol at the beginning of the simulation and identifies the shortest delay path between a producer and consumer. Therefore, with no congestion 

%--------------------------
\subsection{Handling the re-transmitted packets}
%In our ndnSIM simulation experiments, 
We set the \textit{maximum re-transmission timeout} of consumers to be $1~S$. That means, the consumer will wait maximum $1s$ before re-transmitting an interest packet for which it did not receive any data packet. In this setting, every time an interest packet is re-transmitted, the expiry time of the corresponding PIT entry in consumer gets extended. Since the lifetime of a PIT entry is $2s$, all the PIT entries of the unsatisfied interests in consumer remain alive until satisfied by data packets. However, the concept of re-transmission and activeness of PIT entry is different in intermediate NDN routers. In a NDN router, an interest packet is considered re-transmitted when there exists an unexpired out-record in the PIT entry of that interest. That means, that interest has been forwarded earlier through some interface, but has not been satisfied yet. If the router forwards that interest again through the same interface or another interface, then the lifetime of PIT entry gets extended. But the PIT entry of that interest may expire and get deleted if no interest with the same name and selector is received by the router or the PIT entry is satisfied within its lifetime. Therefore, even if an interest is a re-transmitted packet from the consumers point of view, it may be considered as new interest packet in the router when no PIT entry exists for the interest. 
There are two ways we can handle re-transmitted packets: 
% \begin{enumerate}
% \item \textbf{BR-way of re-transmission:} Consider the interest as a re-transmitted packet and forward it in the same way as BestRoute (BR) does. To forward a re-transmitted interest, BR strategy first tries to find an unused interface. If it can not not find any unused interface, then it uses an interface that has been used earliest.
% \item \textbf{Non-BR-way of re-transmission:} Consider the interest as new packet and forward it through any of the interfaces chosen by the agent.
% \end{enumerate}
(i) {BR-way:} We forward the re-transmitted packet in the same way as the BestRoute (BR) algorithm does. To forward a re-transmitted interest, BR strategy first tries to find an unused interface. If it can not not find any unused interface, then it uses an interface that has been used immediately before.
(ii) {Reward as a function of Re-transmission} We consider the re-transmitted packet as new packet and forward it through an interfaces recommended by the agent.

To evaluate which method of re-transmission is better we conducted an experiment where the average delay of the last $5$ packets and interest satisfaction ratio of each interface were considered as the state vector. The reward was chosen to minimize the average of delays of the data packets received through the last chosen interface between last decision epoch and current decision epoch ($\alpha = 0$). We trained the agents for $50$ episodes with $\delta t = 20$, batch size = 16, and learning rate = 1. In order to simplify the learning task we restricted the number of available next hop interface in FIB (Forwarding Information Base) for each node to $2$. 
\subsubsection{BR-way of re-transmission}
The results with BR-way of re-transmission are summarized in Table~\ref{tab:BR-D-st} for three different interest rates (100, 300, and 500, packets/sec).
%The results with both the ways of re-transmission are summarized in Table~\ref{tab:BR-D-st} and 
%-------------------------
%--------------------------
% \subsubsection{BR-way of re-transmission}
% \label{BR-D-st}
% We performed experiments %on topology of Figure~\ref{fig:topo-Sprint-2} 
% with three different interest rates (100, 300, and 500, packets/sec) using the following experiment setup. 
% We used average delay of the last 5 packets and interest satisfaction ratio per interface as state feature. We define the reward to optimize as average of delays of the data packets received through the last chosen interface between last decision epoch and current decision epoch.  Trained the agents using epsilon-greedy method for $50$ episodes with $\delta t = 20$, batch size = 16, and learning rate = 1. Number of available next hop interface in FIB (Forwarding Information Base) per node were restricted to 2 during training. The results are summarized in Table~\ref{tab:BR-D-st}.
%---------summary-----------
\begin{table}[h!]
  \begin{center}
    \begin{tabular}{|l|l|l|l|l|} % 
    \hline
    \textbf{Interest Rate} & \multicolumn{2}{c|}{\textbf{Total}} & \multicolumn{2}{c|}{\textbf{Avg App}} \\
    \textbf{(pkts/s)} & \multicolumn{2}{c|}{\textbf{Throughput (Mbps)}} & \multicolumn{2}{c|}{\textbf{Delay (ms)}}\\
      \hline
      & BR & RL & BR & RL\\
      \hline
      300 & 1.65 & 1.65 & 1140.68 & 1135.40\\
      \hline
      500 & 1.29 & 1.34 & 2606.40 & 2211.68\\
      \hline
    %   1000 & 1.30 & 1.33 & 4853.65 & 4309.31\\
    %   \hline
    \end{tabular}
    \caption{BR-D-st: Summary results}
    \label{tab:BR-D-st}
  \end{center}
\end{table}
%--------------------------
We found that the total throughput and average delay of both BR and RL strategies remained same. All the four node agents use the minimum delay next hop interface for transmitting the new packets. 

With 300 interest rate the maximum number of re-transmissions per packet from the consumer was one. So BR strategy used only the second ranked next hop interface to forward those packets. Since RL strategy in this experiment utilizes the same mechanism to forward re-transmitted packets, the total throughput and average delay for BR and RL are almost same.  

For $500$ packets/sec, the congestion increases and we observe that the total throughput of RL strategy is $12.4\%$ higher compared to BR strategy. Similarly the average delay of RL strategy is $15.14\%$ lower than that of BR strategy. This is because the BR strategy used some alternate next hop interfaces to forward re-transmitted packets, which causes the data packets to either drop or travel through a longer delay path. For example, Chicago sent some interest packets to Stockton and Kansas City. On the contrary, RL strategy was forced to use only two next hop interfaces. Thus, RL strategy got a small advantage in gaining improved throughput and delay. 

% %-----------------------------
% \subsubsection{300 packets per second ($\approx 2.45~Mbps$)}

% We present the results of this experiment in Figures \vrefrange {fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-performance}{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-nodestat}.
% From Figure~\ref{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-performance}, we find that the total throughput and average delay of both BR and RL strategies are same. Figure~\ref{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-nodestat} shows us that all the four node agents use the minimum delay next hop interface for transmitting the new packets. 
% With 300 interest rate the maximum number of re-transmissions per packet from the consumer is one. So BR strategy uses only the second ranked next hop interface to forward those packets. Since RL strategy in this experiment utilizes the same mechanism to forward re-transmitted packets, the total throughput and average delay for BR and RL are almost same.   

% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-app-delay.pdf}
% \caption{Network Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-app-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--throughput}
% \end{subfigure}
% \caption{BR-D-st:Network Performance 300 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-performance}
% \end{figure}

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60/RW0-Rt300-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300--Node4}
% \end{subfigure}
% \caption{BR-D-st:Node statistics for 300 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r300l60-ld50sr300sd60RW0-Rt300-nodestat}
% \end{figure}

% %----------------------
% \subsubsection{500 packets per second ($\approx 4~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-performance}{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-nodestat}. In this experiment, we observe that the total throughput of RL strategy is 12.4\% higher compared to BR strategy. Similarly the average delay of RL strategy is 15.14\% lower than that of BR strategy. This is because the BR strategy used some alternate next hop interfaces to forward re-transmitted packets, which causes the data packets to either drop or travel through a longer delay path. For example, Chicago sent some interest packets to Stockton and Kansas City. On the contrary, RL strategy was forced to use only two next hop interfaces. Thus, RL strategy gets slight advantage in gaining better throughput and delay. 

% %-----------------
% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-app-delay.pdf}
% \caption{Network Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-app-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--throughput}
% \end{subfigure}
% \caption{BR-D-st:Network Performance 500 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-performance}
% \end{figure}

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60/RW0-Rt500-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500--Node4}
% \end{subfigure}
% \caption{BR-D-st:Node statistics for 500 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r500l60-ld50sr500sd60RW0-Rt500-nodestat}
% \end{figure}
% %----------------------------
% %====================
% \subsubsection{1000 packets per second ($\approx 8~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-performance}{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-nodestat}. We observe that with 1000 interest rate RL strategy 
% achieves 14.62\% higher total throughput and 13.86\% lower average delay compared to BR strategy. The is because unlike BR strategy, the RL strategy forwards some new packets through alternative next hop interface instead of using only the minimum delay next hop interface. As a result, in RL strategy packet drops are slightly less than that of BR strategy.    

% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-app-delay.pdf}
% \caption{Network Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-app-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-throughput.pdf}
% \caption{Throughput}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--throughput}
% \end{subfigure}
% \caption{BR-D-st:Network Performance 1000 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-performance}
% \end{figure}

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Aug18/BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0/RW0-Rt1000-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000--Node4}
% \end{subfigure}
% \caption{BR-D-st:Node statistics for 1000 interest rate}
% \label{fig:BR-D-st-TnTDQN-W32NFR-20-e50r1000l60-ld50sr1000sd60rt=0RW0-Rt1000-nodestat}
% \end{figure}

%---------------------------
\emph{Is BR-way of re-transmission good? :}
One of the problems with BR way of re-transmission is that it may sometimes forward interests through an unused next hop interface which goes along a longer path. Moreover, BR strategy always forwards all new packets to the lowest ranked next hop interface whereas sometimes it is useful to distribute some of the new packets as well as re-transmitted packets to alternate interfaces. If RL strategy follows this mechanism, then there is very little scope for the agent to learn how to distribute the packets in other interfaces. Specially, when interest rate is high, the number of re-transmitted interest packets increase. As a result, the agents will not have enough data for training.    
%=============================
%\subsubsection{Re-transmission as feature}
\subsubsection{Reward as a function of re-transmission}
The motivation to define this feature is to capture the congested situation of a path in the network. Since packets are usually re-transmitted when consumer does not receive data within a specific time, we can use the re-transmission feature to represent the congestion that exists for a next hop interface. Let us represent the re-transmission feature as: 

$\mathbf{R}_t^n = [r_1^n, r_2^n, \cdots r_F^n]$, where $F$ is the number of interfaces available at node $n$ and $r_j^n$ is the re-transmission value for the $j$-th interface at node $n$. When $j$-th interface is chosen in the last decision epoch, re-transmission value can be computed in the following two ways:
    
\begin{enumerate}
    \item Re-transmission ratio:  
    \begin{equation}
    \label{eq:rr}
        r_j^n=
        \begin{cases}
        0, & \text{if}\ R_j<=0 \\
        R_j/R, & \text{otherwise}
        \end{cases}
    \end{equation}
    ,where $R_j$ is the number of packets that were originally transmitted through interface $j$, but re-transmitted through $j$ in the last decision epoch, and $R$ is the total number of re-transmitted packets through $j$ in the last decision epoch. 
     \item Re-transmission difference: 
     \begin{equation}
     \label{eq:rd}
        r_j^n=
        \begin{cases}
        0, & \text{if}\ R-N<0 \\
        R-N, & \text{otherwise}
        \end{cases}
    \end{equation}
    ,where $N$ is the number of new packets transmitted through $j$ in the last decision epoch.
\end{enumerate}
%---------------------
\begin{figure}[ht]
  \centering
  %\includegraphics[scale=.5]{figures/rt_feature.pdf}
  \includegraphics[width=\columnwidth]{figures/rt_feature.pdf}
  \caption{Re-transmission as feature}
  \label{fig:re-transmission feature}
\end{figure}
%------------------------
We illustrate the above terms in Figure~\ref{fig:re-transmission feature}. Let us assume that at time $t$ we need to get a decision from the node agent. In the last decision epoch at time $t-\delta t$, the predicted interface was \textit{Face1}. Assume that among all the packets transmitted between $t$ and $t-\delta t$ through \textit{Face1}, four packets were re-transmitted packets and one packet was a new packet, i.e. $R = 4$ and $N=1$. If out of four packets, three packets were originally transmitted (new) through \textit{Face1} at time $(t-101\times\delta t)$ and one packet was originally transmitted (new) through \textit{Face2} at time $t-103\delta t$, then $R_1 = 3$, $R_2 = 1$, and $R=R_1+R_2$. Now, according to equation \ref{eq:rr}, $r_1^n = 3/4 = 0.75$ and
according to equation \ref{eq:rd},  $r_1^n = 4-1 = 3$.
%----------------------
%=============================
%\clearpage
%\newpage
%========RW-1-2==============
\subsubsection{Non-BR-way of re-transmission} %\textcolor{red}{BEST RESULTS: Reward-1-2}}
\label{NBR-RW1-2}

For this case, we used re-transmission difference in Equation \ref{eq:rd} as extra feature of the state along with the average delay and interest satisfaction ratio features. We chose the reward as: 
    \small
    \begin{equation}
    \label{eq:rw1}
        RW1 =
        \begin{cases}
         -(AvgD + R_{lf}\times CM)    , & \text{if}\ R-N > R_{thrs} \: \text{and} \: AvgD \ne 0 \\
         -(R_{lf}\times CM)    , & \text{if}\ R-N > R_{thrs} \: \text{and} \: AvgD = 0 \\
         -(AvgD), & \text{if}\ R-N \leq R_{thrs} \: \text{and} \: AvgD \ne 0 \\
        -10000, & \text{if}\ R-N \leq R_{thrs} \: \text{and} \: AvgD = 0 
        \end{cases}
    \end{equation}
    \normalsize
to minimize the overall delay in the network.
 where $lf$ is the chosen interface in the last decision epoch, $R_{lf}$ is the number of packets in $R$ which were transmitted through $lf$ last time, $AvgD$ is average delay of the data packets received through interface $lf$ between last decision epoch and current decision epoch, $CM$ is a constant multiplier to make the reward smaller to account for the re-transmitted packets due to packet drops, $R=$ number of
    re-transmitted packets and $N=$ number of new packets in the last decision epoch, $R_{thrs}$ is a threshold. We chose $R_{thrs}=0$ for 300 interest rate and $R_{thrs}=1$ for 500 interest rate, and $R_{thrs}=2$ for 1000 interest rate. In our experiment, we chose different values of $CM \in \{ 1000, 4000, 8000, 20000\}$ and present the results of $CM=4000$. Number of available next hop interface per node were restricted to 2 during training. Trained for 50 episodes with $\delta t = 10$, batch size = 16, and learning rate = 1. We summarize the results in Table~\ref{tab:RD-st-p4s}.

% We performed experiments on topology of Figure~\ref{fig:topo-Sprint-2} with three different interest rates (300, 500, and 1000 packets/sec) using the following experiment setup.  

% \begin{enumerate}
%     \item \textcolor{blue}{Used re-transmission difference in Equation \ref{eq:rd} as extra feature of the state along with the average delay and interest satisfaction ratio features.}
    
%     \item Goal is to minimize the overall delay in the network.
    
%     \item 
%     The reward function for interface $lf$ is the following,
%     \small
%     \begin{equation}
%     \label{eq:rw1}
%         RW1 =
%         \begin{cases}
%          -(AvgD + R_{lf}\times CM)    , & \text{if}\ R-N > R_{thrs} \: \text{and} \: AvgD \ne 0 \\
%          -(R_{lf}\times CM)    , & \text{if}\ R-N > R_{thrs} \: \text{and} \: AvgD = 0 \\
%          -(AvgD), & \text{if}\ R-N \leq R_{thrs} \: \text{and} \: AvgD \ne 0 \\
%         -10000, & \text{if}\ R-N \leq R_{thrs} \: \text{and} \: AvgD = 0 
%         \end{cases}
%     \end{equation}
%     \normalsize
%      where $lf$ is the chosen interface in the last decision epoch, $R_{lf}$ is the number of packets in $R$ which were transmitted through $lf$ last time, $AvgD$ is average delay of the data packets received through interface $lf$ between last decision epoch and current decision epoch, $CM$ is a constant multiplier to make the reward smaller to account for the re-transmitted packets due to packet drops, $R=$ number of
%     re-transmitted packets and $N=$ number of new packets in the last decision epoch, $R_{thrs}$ is a threshold. We chose $R_{thrs}=0$ for 300 interest rate and $R_{thrs}=1$ for 500 interest rate, and $R_{thrs}=2$ for 1000 interest rate. In our experiment, we chose different values of $CM \in \{ 1000, 4000, 8000, 20000\}$ and present the results of $CM=4000$. %in Figures \vrefrange {fig:Time2TDQN-SW32-NoFlowRFace-10-e50r300l60-load20sr300sd180rt=0-tlr=500_perform}{fig:Time2TDQN-SW32-NoFlowRFace-10-e50r500l60-load30sr500sd180rt=1-tlr=500_nodestat}. 
    
%     \item Used Non-BR-way of re-transmission to handle re-transmitted packets. 
    
%     \item Number of available next hop interface per node were restricted to 2 during training.
    
%     \item Trained the agents using epsilon-greedy method for multiple episodes.
    
%     \item Trained for 50 episodes with $\delta t = 10$, batch size = 16, and learning rate = 1. 
    
%     \item  We summarize the results in Table~\ref{tab:RD-st-p4s}.
% \end{enumerate}

%-------------------------
\begin{table}[h!]
  \begin{center}
    \begin{tabular}{|l|l|l|l|l|} % 
    \hline
    \textbf{Interest Rate} & \multicolumn{2}{c|}{\textbf{Total}} & \multicolumn{2}{c|}{\textbf{Avg App}} \\
    \textbf{(pkts/s)} & \multicolumn{2}{c|}{\textbf{Throughput (Mbps)}} & \multicolumn{2}{c|}{\textbf{Delay (ms)}}\\
      \hline
      & BR & RL & BR & RL\\
      \hline
      300 & 1.69 & 1.44 & 1148.42 & 1340.29 \\
      \hline
      500 & 1.31 & 1.75 & 2691.18 & 2121.94\\
      \hline
    %   1000 & 1.31 & 1.30 & 5370.49 & 5963.16 \\
    %   \hline
    \end{tabular}
    \caption{RD-st-p4s: Summary results of RW1}
    \label{tab:RD-st-p4s}
  \end{center}
\end{table}

%--------300------------------
For a data rate of $300$ packets/sec, we find that after 20 seconds of simulation, node agent Cheyenne forwards interest packets 60\%-80\% times through Stockton, the minimum delay next hop and 20\%-40\% times through the KansasCity next hop. The more utilization of the minimum delay next hop and less utilization of the alternate next hop interface causes the RL strategy to achieve total throughput of 1.44 Mbps, which is 6.67\% better than what we achieved when we used the Equation \ref{eq:rr} to compute the re-transmission feature. We conjecture that Equation \ref{eq:rd} better represents the congested state of the network and facilitates frequent switching of the links. Because in Equation \ref{eq:rd}, we are assigning a higher value, $R-N$ to the last chosen interface. That means, we are forwarding more re-transmitted packets and most probably that interface will become congested. On the other hand, in Equation \ref{eq:rr} we assign $R_{lf}$ value which represents a 1 second older congested state of the last chosen interface. 

For a data rate of $300$ packets/sec, we observe that node agent Cheyenne keep switching links from the beginning of the simulation. The almost even utilization of the both Stockton and KansasCity next hop interfaces allowed the RL strategy to achieve total throughput of 1.75 Mbps, which is 33.59\% higher than BR strategy and 8\% better than what we achieved when we used the Equation \ref{eq:rr} to compute the re-transmission feature. We speculate that because of the higher interest rate the number of re-transmissions are higher in this case. As a result, in Equation \ref{eq:rd} the assigned $R-N$ values are higher most of the time. This helps the agent to alternate links frequently considering the congested state of the next hop interfaces. 

% \subsubsection{300 packets per second ($\approx 2.45~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-performance}{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-debug-rtt-pnlt-summ}.

% From Figure~\ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node3}
% we find that after 20 seconds of simulation, node agent Cheyenne forwards interest packets 60\%-80\% times through Stockton, the minimum delay next hop and 20\%-40\% times through the KansasCity next hop. The more utilization of the minimum delay next hop and less utilization of the alternate next hop interface causes the RL strategy to achieve total throughput of 1.44 Mbps, which is 6.67\% better than what we achieved when we used the Equation \ref{eq:rr} to compute the re-transmission feature. We conjecture that Equation \ref{eq:rd} better represents the congested state of the network and facilitates frequent switching of the links. Because in Equation \ref{eq:rd}, we are assigning a higher value, $R-N$ to the last chosen interface. That means, we are forwarding more re-transmitted packets and most probably that interface will become congested. On the other hand, in Equation \ref{eq:rr} we assign $R_{lf}$ value which represents a 1 second older congested state of the last chosen interface. 

%-------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-net-delay.pdf}
% \caption{Network Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-net-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-net-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-net-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--throughput}
% \end{subfigure}
% \caption{RD-st-p4s:Network Performance 300 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-performance}
% \end{figure}
% %-------------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300--Node4}
% \end{subfigure}
% \caption{RD-st-p4s:Node statistics for 300 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-nodestat}
% \end{figure}
%-----------------debugging---------
% \begin{figure}[h!]
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Cheyenne-rtt-pnlt-summ.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-Node3-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-KansasCity-rtt-pnlt-summ.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-Node6-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Stockton-rtt-pnlt-summ.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-Node9-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0/RW1-Rt300-Chicago-rtt-pnlt-summ.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-Node4-rtt-pnlt-summ}
% \end{subfigure}
% \caption{RD-st-p4s:Time vs Condition Satisfied for 300 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r300l60-ld50sr300sd180rt=0RW1-Rt300-debug-rtt-pnlt-summ}
% \end{figure}

% %--------------500--------------
% \subsubsection{500 packets per second ($\approx 4~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-performance}{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-debug-rtt-pnlt-summ}.

% From Figure~\ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node3}
% we observe that node agent Cheyenne keep switching links from the beginning of the simulation. The almost even utilization of the both Stockton and KansasCity next hop interfaces allowed the RL strategy to achieve total throughput of 1.75 Mbps, which is 33.59\% higher than BR strategy and 8\% better than what we achieved when we used the Equation \ref{eq:rr} to compute the re-transmission feature. We speculate that because of the higher interest rate the number of re-transmissions are higher in this case. As a result, in Equation \ref{eq:rd} the assigned $R-N$ values are higher most of the time. This helps the agent to alternate links frequently considering the congested state of the next hop interfaces. 

% %-----------------
% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-net-delay.pdf}
% \caption{Network Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-net-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-net-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-net-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--throughput}
% \end{subfigure}
% \caption{RD-st-p4s:Network Performance 500 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-performance}
% \end{figure}
% %--------------------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500--Node4}
% \end{subfigure}
% \caption{RD-st-p4s:Node statistics for 500 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-nodestat}
% \end{figure}
%-----------------debugging---------
% \begin{figure}[h!]
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Cheyenne-rtt-pnlt-summ.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-Node3-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-KansasCity-rtt-pnlt-summ.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-Node6-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Stockton-rtt-pnlt-summ.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-Node9-rtt-pnlt-summ}
% \end{subfigure}
% \begin{subfigure}{0.9\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1/RW1-Rt500-Chicago-rtt-pnlt-summ.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-Node4-rtt-pnlt-summ}
% \end{subfigure}
% \caption{RD-st-p4s:Time vs Condition Satisfied for 500 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e50r500l60-ld50sr500sd180rt=1RW1-Rt500-debug-rtt-pnlt-summ}
% \end{figure}

%----------1000-----------------
% \subsubsection{1000 packets per second ($\approx 8~Mbps$)}
% %\label{subsubsec:2}
% We present the results of this experiment in Figures \vrefrange {fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-performance}{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-debug-rtt-pnlt-summ}.

% From Figure~\ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node3}, \ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node4}, and \ref{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node9}, we find that from the beginning of the simulation, node agents Cheyenne, Stockton, and Chicago forward interest packets through both of their next hop interfaces. Because of the higher interest rate, experience replay memory fills up with transition samples from both hops. Since lots of re-transmissions occur in all three nodes and the reward is defined as a function of the number of re-transmissions, the DQN network of the nodes update their parameters frequently. Moreover, in Equation \ref{eq:rd} the assigned $R-N$ values are higher most of the time, which also helps the agent to capture the congested state of the next hops and alternate links. Due to the higher data rate lots of packets drop at Stockton and Chicago in addition to Seattle. Therefore, the throughput oscillates between 0.9 Mbps and 1.7 Mbps.
% %----------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.45\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-net-delay.pdf}
% \caption{Network Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-net-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-net-delay-cdf.pdf}
% \caption{Network Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-net-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-app-delay-cdf.pdf}
% \caption{Application Delay CDF}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-app-delay-cdf}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-throughput.pdf}
% \caption{Throughput}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--throughput}
% \end{subfigure}
% \caption{RD-st-p4s:Network Performance 1000 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-performance}
% \end{figure}
% %------------------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-Cheyenne-link-util.pdf}
% \caption{Cheyenne}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node3}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-KansasCity-link-util.pdf}
% \caption{Kansas City}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node6}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-Stockton-link-util.pdf}
% \caption{Stockton}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node9}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Sep28/RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2/RW1-Rt1000-Chicago-link-util.pdf}
% \caption{Chicago}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000--Node4}
% \end{subfigure}
% \caption{RD-st-p4s:Node statistics for 1000 interest rate}
% \label{fig:RD-st-p4s-T2TDQN-W32NFR-10-e40r1000l60-ld40sr1000sd180rt=2RW1-Rt1000-nodestat}
% \end{figure}
%--------------------------
\subsubsection{\textcolor{blue}{Training duration (short vs long)}}
In this experiment, we compared the performance of two RL models trained with different lengths of simulation. We trained each model for $50$ episodes with $60$ and $500$ seconds per episode. %In Figure~\ref{fig:RD-st-p4s-500-Short-Long-performance}, \textit{RL-Ep50-L60} refers to the model which has been trained 60 seconds per episode and \textit{RL-Ep50-L500} refers to the model which has been trained $500$ seconds per episode. 
%--------500----------
If we compute the total throughput and average delay for the steady state of the network, i.e. ignoring the data of first 20 seconds of simulation, %we find that \textit{RL-Ep50-L60} 
we found that the model trained for $60$ seconds/episodes achieves $7.2\%$ higher throughput and $6.4\%$ less average application delay compared to the model trained for $500$ seconds/episodes. %\textit{RL-Ep50-L500} model.  
%--------300--------
%If we compute the total throughput and average delay for the steady state of the network, i.e. ignoring the data of first 20 seconds of simulation, we find that \textit{RL-Ep50-L60} model achieves 3.4\% higher throughput and 10.49\% less average application delay compared to the \textit{RL-Ep50-L500} model.  


% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:Multi-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:Multi-Rt500-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 500 interest rate (Short vs Long duration)}
% \label{fig:RD-st-p4s-500-Short-Long-performance}
% \end{figure}

% %-----------300----------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:Multi-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:Multi-Rt300-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 300 interest rate (Short vs Long duration)}
% \label{fig:RD-st-p4s-300-Short-Long-performance}
% \end{figure}

%----------------------
\subsubsection{\textcolor{blue}{One vs Multi Episode Training:}}

In this experiment, we compare performance of two RL models, one trained with $50$ episodes of $60$ seconds  duration and another with one episode of $6000$ seconds duration. Comparing the steady state (discarding first 20 seconds of simulation) data, We observed that the model with $50$ episodes achieves $33.6\%$ higher throughput and 25.4\% less application delay compared to the model with one long episode.
%In Figure~\ref{fig:RD-st-p4s-One-Multi-performance}, \textit{RL-Ep50-L60} refers to the model which has been trained for 50 episodes where duration of each episode was 60 seconds and \textit{RL-Ep1-L6000} refers to the model which has been trained for one episode where duration of the single episode was 6000 seconds. Computing the total throughput and average delay for the steady state of the network (discarding first 20 seconds of simulation data), we find that \textit{RL-Ep50-L60} model achieves 33.6\% higher throughput and 25.4\% less application delay compared to the \textit{RL-Ep1-L6000} model.   

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-vs-One-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:Multi-vs-One-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-vs-One-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:Multi-vs-One-Rt500-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 500 interest rate (One vs Multi Episode)}
% \label{fig:RD-st-p4s-One-Multi-performance}
% \end{figure}

% %---------------300-----------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-vs-One-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:Multi-vs-One-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/Multi-vs-One-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:Multi-vs-One-Rt300-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 300 interest rate (One vs Multi Episode)}
% \label{fig:RD-st-p4s-300-One-Multi-performance}
% \end{figure}

%---------------
\subsubsection{\textcolor{blue}{Low vs High learning rate:}}

In this experiment, we compare performance of two RL strategy models tested with different learning rates \textcolor{red}{is it the Q-value update learning rate or the DNN weight update learning rate}. We chose two learning rates of $100$ and $500$. These values were chosen by a trial-and-error approach. %In Figure~\ref{fig:RD-st-p4s-300-Low-High-performance}, \textit{Ep50-L60-LR100} refers to the model which has been tested with learning rate $100$ and \textit{Ep50-L60-LR500} refers to the model which has been tested with learning rate 500. 
Both models were trained for $50$ episodes with $60$ seconds of simulation per episode. Comparing the steady state performance we observed that the model with a learning rate of $500$ achieves $38.53\%$ higher throughput and $57.47\%$ less application delay compared to the model with a learning rate of $100$.
%Computing the total throughput and average delay for the steady state of the network (discarding first 20 seconds of simulation data), we find that \textit{Ep50-L60-LR500} model achieves 38.53\% higher throughput and 57.47\% less application delay compared to the \textit{Ep50-L60-LR100} model. 

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/LearningRate-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:LearningRate-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/LearningRate-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:LearningRate-Rt300-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 300 interest rate (Low vs High Learning rate)}
% \label{fig:RD-st-p4s-300-Low-High-performance}
% \end{figure}

% %----------500--------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/LearningRate-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:LearningRate-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct22/LearningRate-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:LearningRate-Rt500-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 500 interest rate (Low vs High Learning rate)}
% \label{fig:RD-st-p4s-500-Low-High-performance}
% \end{figure}
% %------------------
%\subsubsection{\textcolor{blue}{Heterogeneity between training and deployment:}}
% In this experiment, we compare performance of two RL strategy models tested with different learning rates. In Figure~\ref{fig:RD-st-p4s-300-Same-Different-performance} and Figure~\ref{fig:RD-st-p4s-500-Same-Different-performance}, \textit{Ep50-L60-CG6-LR500} refers to the model which has been trained with learning rate 1 and tested with learning rate 500 and \textit{Ep50-L60-CG5-LR500} refers to the model which has been trained and tested with learning rate 500. Both models were trained for 50 episodes with 60 seconds of simulation per episode. Computing the total throughput and average delay for the steady state of the network (discarding first 20 seconds of simulation data), we find that \textit{Ep50-L60-CG6-LR500} model achieves 13.73\% and 30.51\% higher throughput for 500 and 300 interest rate respectively compared to the \textit{Ep50-L60-CG5-LR500} model. Also, \textit{Ep50-L60-CG6-LR500} model obtains 12.66\% and 28.75\% less application delay for 500 and 300 interest rate respectively compared to the \textit{Ep50-L60-CG5-LR500} model. 

% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct27/LR2-Rt300-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:LearningRate2-Rt300-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct27/LR2-Rt300-throughput.pdf}
% \caption{Throughput}
% \label{fig:LearningRate2-Rt300-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 300 interest rate (Same vs Different Learning rate)}
% \label{fig:RD-st-p4s-300-Same-Different-performance}
% \end{figure}

% %----------500--------------
% \begin{figure}[h!]
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct27/LR2-Rt500-app-delay.pdf}
% \caption{Application Delay}
% \label{fig:LearningRate2-Rt500-app-delay}
% \end{subfigure}
% \begin{subfigure}{0.4\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/Fig_Oct27/LR2-Rt500-throughput.pdf}
% \caption{Throughput}
% \label{fig:LearningRate-Rt500-throughput}
% \end{subfigure}
% \caption{RD-st-p4s: Network Performance 500 interest rate (Same vs Different Learning rate)}
% \label{fig:RD-st-p4s-500-Same-Different-performance}
% \end{figure}

%==========================



%--------------------------
\begin{figure}[htbp]
  \centering
  %\includegraphics[width=\textwidth,height=8cm]{figures/sprint2-wcp.pdf}
  \includegraphics[scale=0.6]{figures/sprint-2-ann.pdf}
  %\includegraphics[scale=.5]{figures/SPRINT_marked_v1.pdf}
  \caption{Sprint topology} 
  \label{fig:topo-Sprint-2}
\end{figure}

\subsection{\textcolor{blue}{Comparison with BR}}
We trained RL strategy model for 500 interest rate and tested that model with simulations of different interest rates. The model was trained for 50 episodes with 60 seconds of simulation per episode.  In Figure~\ref{fig:RD-st-p4s-500-model-test} we show the percentage improvement of throughput and average application delay for different interest rates compared to \emph{bestroute} strategy. We found that when the data rate is almost double (3.3$\sim$4 Mbps) the capacity (2 Mbps) of the network, only then we get 16\%-30\% increase in throughput and 9\%-19\% decrease in average application delay compared to bestroute. When data rate is lower or close to 2 Mbps, in those cases performance degrades 46\%-117\%. 

\begin{figure}[h!]
\includegraphics[width=\linewidth]{figures/RateComp.pdf}
\caption{RD-st-p4s: Network Performance of different interest rates with One trained model}
\label{fig:RD-st-p4s-500-model-test}
\end{figure}
%------------------

==> related_work.tex <==
\section{Related work}
